Divergence based Ranked Preference Alignment for LLMs

Alignment of large language models typically relies on pairwise preference feedback, though ranked feedback can capture more comprehensive information across multiple responses within a single annotation. However, ranked-preference alignment is underexplored in practice compared to simpler pairwise approaches, potentially resulting in suboptimal behavior. Concurrently, recent research has conceptualized large language model alignment objectives as divergence estimators between aligned (preferred) and unaligned (less-preferred) response distributions, resulting in a family of objectives with an interpretable theoretical foundation and strong empirical performance. This work unifies these perspectives by introducing $f$-RPO, a $f$-divergence objective for ranked preference optimization that extends divergence-based alignment to ranked feedback and recovers pairwise preference alignment as a special case. Our theoretical analysis establishes rank-order consistency, showing that $f$-RPO preserves the underlying preference ordering at convergence. Empirical results indicate that total-variation and reverse-KL variants of the proposed objective consistently outperform ranked-alignment baselines in both ranking and generation quality across Qwen, Llama, & Gemma models ranging from 0.5B to 8B parameters.

==> scaling_table_across_methods.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Method & Model & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
\multirow{3}{*}{Baseline} & 0.5B & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} \\
 & 1.5B & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} \\
 & 7B & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} \\
\midrule
\multirow{3}{*}{Mallows-RCPO} & 0.5B & \shortstack{$\rho$: 0.1650 $\pm$ 0.0025 \\ Top-1: \textbf{0.2897 $\pm$ 0.0029}} & \shortstack{$\rho$: 0.1634 $\pm$ 0.0036 \\ Top-1: \textbf{0.2881 $\pm$ 0.0031}} & \shortstack{$\rho$: 0.1655 $\pm$ 0.0054 \\ Top-1: \textbf{0.2887 $\pm$ 0.0034}} & \shortstack{$\rho$: 0.1659 $\pm$ 0.0054 \\ Top-1: \textbf{0.2891 $\pm$ 0.0033}} \\
 & 1.5B & \shortstack{$\rho$: 0.0646 $\pm$ 0.0080 \\ Top-1: 0.2487 $\pm$ 0.0044} & \shortstack{$\rho$: 0.0620 $\pm$ 0.0056 \\ Top-1: 0.2496 $\pm$ 0.0007} & \shortstack{$\rho$: 0.0688 $\pm$ 0.0184 \\ Top-1: 0.2497 $\pm$ 0.0027} & \shortstack{$\rho$: 0.0665 $\pm$ 0.0143 \\ Top-1: 0.2491 $\pm$ 0.0037} \\
 & 7B & \shortstack{$\rho$: 0.5128 $\pm$ 0.0053 \\ Top-1: \textbf{0.3347 $\pm$ 0.0029}} & \shortstack{$\rho$: 0.5084 $\pm$ 0.0095 \\ Top-1: \textbf{0.3324 $\pm$ 0.0093}} & \shortstack{$\rho$: 0.5051 $\pm$ 0.0200 \\ Top-1: \textbf{0.3329 $\pm$ 0.0084}} & \shortstack{$\rho$: 0.5080 $\pm$ 0.0078 \\ Top-1: \textbf{0.3317 $\pm$ 0.0070}} \\
\midrule
\multirow{3}{*}{PL-DPO} & 0.5B & \shortstack{$\rho$: 0.1321 $\pm$ 0.0031 \\ Top-1: 0.2597 $\pm$ 0.0011} & \shortstack{$\rho$: 0.1422 $\pm$ 0.0046 \\ Top-1: 0.2537 $\pm$ 0.0019} & \shortstack{$\rho$: 0.1543 $\pm$ 0.0064 \\ Top-1: 0.2558 $\pm$ 0.0023} & \shortstack{$\rho$: 0.1555 $\pm$ 0.0053 \\ Top-1: 0.2553 $\pm$ 0.0019} \\
 & 1.5B & \shortstack{$\rho$: 0.0424 $\pm$ 0.0031 \\ Top-1: 0.2244 $\pm$ 0.0040} & \shortstack{$\rho$: 0.0571 $\pm$ 0.0041 \\ Top-1: 0.2289 $\pm$ 0.0045} & \shortstack{$\rho$: 0.0747 $\pm$ 0.0065 \\ Top-1: 0.2352 $\pm$ 0.0038} & \shortstack{$\rho$: 0.0785 $\pm$ 0.0058 \\ Top-1: 0.2375 $\pm$ 0.0028} \\
 & 7B & \shortstack{$\rho$: 0.4862 $\pm$ 0.0026 \\ Top-1: \underline{0.3208 $\pm$ 0.0039}} & \shortstack{$\rho$: 0.4905 $\pm$ 0.0024 \\ Top-1: \underline{0.3144 $\pm$ 0.0045}} & \shortstack{$\rho$: 0.4950 $\pm$ 0.0015 \\ Top-1: \underline{0.3165 $\pm$ 0.0040}} & \shortstack{$\rho$: 0.4945 $\pm$ 0.0023 \\ Top-1: \underline{0.3171 $\pm$ 0.0029}} \\
\midrule
\multirow{3}{*}{f-RPO-TV} & 0.5B & \shortstack{$\rho$: \underline{0.2010 $\pm$ 0.0059} \\ Top-1: \underline{0.2737 $\pm$ 0.0033}} & \shortstack{$\rho$: \underline{0.2115 $\pm$ 0.0050} \\ Top-1: \underline{0.2712 $\pm$ 0.0014}} & \shortstack{$\rho$: \textbf{0.2137 $\pm$ 0.0045} \\ Top-1: \underline{0.2704 $\pm$ 0.0022}} & \shortstack{$\rho$: \textbf{0.2128 $\pm$ 0.0031} \\ Top-1: \underline{0.2694 $\pm$ 0.0027}} \\
 & 1.5B & \shortstack{$\rho$: \underline{0.1356 $\pm$ 0.0100} \\ Top-1: \underline{0.2605 $\pm$ 0.0054}} & \shortstack{$\rho$: \underline{0.1509 $\pm$ 0.0111} \\ Top-1: \underline{0.2620 $\pm$ 0.0056}} & \shortstack{$\rho$: \underline{0.1539 $\pm$ 0.0074} \\ Top-1: \underline{0.2636 $\pm$ 0.0049}} & \shortstack{$\rho$: \underline{0.1544 $\pm$ 0.0077} \\ Top-1: \underline{0.2648 $\pm$ 0.0051}} \\
 & 7B & \shortstack{$\rho$: \textbf{0.5287 $\pm$ 0.0015} \\ Top-1: 0.3063 $\pm$ 0.0049} & \shortstack{$\rho$: \textbf{0.5278 $\pm$ 0.0019} \\ Top-1: 0.2961 $\pm$ 0.0044} & \shortstack{$\rho$: \textbf{0.5265 $\pm$ 0.0013} \\ Top-1: 0.2948 $\pm$ 0.0022} & \shortstack{$\rho$: \textbf{0.5260 $\pm$ 0.0013} \\ Top-1: 0.2940 $\pm$ 0.0034} \\
\midrule
\multirow{3}{*}{f-RPO reverse KL} & 0.5B & \shortstack{$\rho$: \textbf{0.2020 $\pm$ 0.0059} \\ Top-1: 0.2683 $\pm$ 0.0016} & \shortstack{$\rho$: \textbf{0.2153 $\pm$ 0.0054} \\ Top-1: 0.2650 $\pm$ 0.0047} & \shortstack{$\rho$: \underline{0.2035 $\pm$ 0.0069} \\ Top-1: 0.2601 $\pm$ 0.0020} & \shortstack{$\rho$: \underline{0.2027 $\pm$ 0.0070} \\ Top-1: 0.2607 $\pm$ 0.0007} \\
 & 1.5B & \shortstack{$\rho$: \textbf{0.1666 $\pm$ 0.0100} \\ Top-1: \textbf{0.2730 $\pm$ 0.0062}} & \shortstack{$\rho$: \textbf{0.2013 $\pm$ 0.0027} \\ Top-1: \textbf{0.2789 $\pm$ 0.0009}} & \shortstack{$\rho$: \textbf{0.1779 $\pm$ 0.0149} \\ Top-1: \textbf{0.2726 $\pm$ 0.0049}} & \shortstack{$\rho$: \textbf{0.1740 $\pm$ 0.0162} \\ Top-1: \textbf{0.2712 $\pm$ 0.0070}} \\
 & 7B & \shortstack{$\rho$: \underline{0.5253 $\pm$ 0.0020} \\ Top-1: 0.3019 $\pm$ 0.0034} & \shortstack{$\rho$: \underline{0.5219 $\pm$ 0.0032} \\ Top-1: 0.2972 $\pm$ 0.0026} & \shortstack{$\rho$: \underline{0.5100 $\pm$ 0.0007} \\ Top-1: 0.2972 $\pm$ 0.0020} & \shortstack{$\rho$: \underline{0.5103 $\pm$ 0.0018} \\ Top-1: 0.2981 $\pm$ 0.0014} \\
\bottomrule
\end{tabular}%
}
\caption{Model-scaling results on the train split. Each cell reports Spearman $\rho$ and Top-1 accuracy as mean $\pm$ sample standard deviation across five seeds. Baselines are single deterministic evaluations and therefore have zero reported standard deviation. Bold and underlined values are respectively best and second-best among methods at the same model size and $k$.}
\label{tab:scaling-combined-train}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Method & Model & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
\multirow{3}{*}{Baseline} & 0.5B & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} \\
 & 1.5B & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} \\
 & 7B & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} \\
\midrule
\multirow{3}{*}{Mallows-RCPO} & 0.5B & \shortstack{$\rho$: 0.1300 $\pm$ 0.0049 \\ Top-1: \underline{0.2851 $\pm$ 0.0065}} & \shortstack{$\rho$: 0.1287 $\pm$ 0.0038 \\ Top-1: \underline{0.2835 $\pm$ 0.0062}} & \shortstack{$\rho$: 0.1307 $\pm$ 0.0053 \\ Top-1: \underline{0.2829 $\pm$ 0.0071}} & \shortstack{$\rho$: 0.1315 $\pm$ 0.0051 \\ Top-1: \underline{0.2846 $\pm$ 0.0043}} \\
 & 1.5B & \shortstack{$\rho$: 0.0369 $\pm$ 0.0123 \\ Top-1: 0.2374 $\pm$ 0.0085} & \shortstack{$\rho$: 0.0326 $\pm$ 0.0089 \\ Top-1: 0.2369 $\pm$ 0.0078} & \shortstack{$\rho$: 0.0430 $\pm$ 0.0322 \\ Top-1: 0.2390 $\pm$ 0.0120} & \shortstack{$\rho$: 0.0394 $\pm$ 0.0249 \\ Top-1: 0.2412 $\pm$ 0.0131} \\
 & 7B & \shortstack{$\rho$: 0.4701 $\pm$ 0.0049 \\ Top-1: \underline{0.2976 $\pm$ 0.0078}} & \shortstack{$\rho$: 0.4667 $\pm$ 0.0061 \\ Top-1: \underline{0.3003 $\pm$ 0.0048}} & \shortstack{$\rho$: 0.4548 $\pm$ 0.0281 \\ Top-1: 0.2938 $\pm$ 0.0113} & \shortstack{$\rho$: 0.4674 $\pm$ 0.0052 \\ Top-1: \underline{0.2976 $\pm$ 0.0052}} \\
\midrule
\multirow{3}{*}{PL-DPO} & 0.5B & \shortstack{$\rho$: 0.0967 $\pm$ 0.0050 \\ Top-1: 0.2791 $\pm$ 0.0027} & \shortstack{$\rho$: 0.1031 $\pm$ 0.0047 \\ Top-1: 0.2775 $\pm$ 0.0015} & \shortstack{$\rho$: 0.1104 $\pm$ 0.0045 \\ Top-1: 0.2791 $\pm$ 0.0019} & \shortstack{$\rho$: 0.1131 $\pm$ 0.0037 \\ Top-1: 0.2824 $\pm$ 0.0035} \\
 & 1.5B & \shortstack{$\rho$: 0.0134 $\pm$ 0.0077 \\ Top-1: 0.2293 $\pm$ 0.0059} & \shortstack{$\rho$: 0.0269 $\pm$ 0.0036 \\ Top-1: 0.2336 $\pm$ 0.0073} & \shortstack{$\rho$: 0.0443 $\pm$ 0.0045 \\ Top-1: 0.2407 $\pm$ 0.0030} & \shortstack{$\rho$: 0.0471 $\pm$ 0.0101 \\ Top-1: 0.2466 $\pm$ 0.0066} \\
 & 7B & \shortstack{$\rho$: 0.4441 $\pm$ 0.0037 \\ Top-1: \textbf{0.3014 $\pm$ 0.0035}} & \shortstack{$\rho$: 0.4478 $\pm$ 0.0044 \\ Top-1: \textbf{0.3008 $\pm$ 0.0033}} & \shortstack{$\rho$: 0.4523 $\pm$ 0.0013 \\ Top-1: \textbf{0.3051 $\pm$ 0.0031}} & \shortstack{$\rho$: 0.4530 $\pm$ 0.0013 \\ Top-1: \textbf{0.3046 $\pm$ 0.0031}} \\
\midrule
\multirow{3}{*}{f-RPO-TV} & 0.5B & \shortstack{$\rho$: \underline{0.1405 $\pm$ 0.0061} \\ Top-1: 0.2786 $\pm$ 0.0040} & \shortstack{$\rho$: \underline{0.1477 $\pm$ 0.0056} \\ Top-1: 0.2808 $\pm$ 0.0036} & \shortstack{$\rho$: \underline{0.1499 $\pm$ 0.0059} \\ Top-1: 0.2786 $\pm$ 0.0023} & \shortstack{$\rho$: \underline{0.1492 $\pm$ 0.0039} \\ Top-1: 0.2780 $\pm$ 0.0041} \\
 & 1.5B & \shortstack{$\rho$: \underline{0.1050 $\pm$ 0.0107} \\ Top-1: \underline{0.2623 $\pm$ 0.0082}} & \shortstack{$\rho$: \underline{0.1243 $\pm$ 0.0101} \\ Top-1: \underline{0.2650 $\pm$ 0.0023}} & \shortstack{$\rho$: \underline{0.1297 $\pm$ 0.0093} \\ Top-1: \underline{0.2672 $\pm$ 0.0049}} & \shortstack{$\rho$: \underline{0.1288 $\pm$ 0.0078} \\ Top-1: \underline{0.2672 $\pm$ 0.0053}} \\
 & 7B & \shortstack{$\rho$: \underline{0.4817 $\pm$ 0.0019} \\ Top-1: 0.2867 $\pm$ 0.0035} & \shortstack{$\rho$: \underline{0.4841 $\pm$ 0.0017} \\ Top-1: 0.2829 $\pm$ 0.0036} & \shortstack{$\rho$: \textbf{0.4854 $\pm$ 0.0023} \\ Top-1: 0.2840 $\pm$ 0.0030} & \shortstack{$\rho$: \textbf{0.4858 $\pm$ 0.0012} \\ Top-1: 0.2840 $\pm$ 0.0023} \\
\midrule
\multirow{3}{*}{f-RPO reverse KL} & 0.5B & \shortstack{$\rho$: \textbf{0.1608 $\pm$ 0.0106} \\ Top-1: \textbf{0.2921 $\pm$ 0.0052}} & \shortstack{$\rho$: \textbf{0.1769 $\pm$ 0.0076} \\ Top-1: \textbf{0.2938 $\pm$ 0.0049}} & \shortstack{$\rho$: \textbf{0.1662 $\pm$ 0.0087} \\ Top-1: \textbf{0.2900 $\pm$ 0.0027}} & \shortstack{$\rho$: \textbf{0.1648 $\pm$ 0.0087} \\ Top-1: \textbf{0.2894 $\pm$ 0.0023}} \\
 & 1.5B & \shortstack{$\rho$: \textbf{0.1435 $\pm$ 0.0154} \\ Top-1: \textbf{0.2732 $\pm$ 0.0089}} & \shortstack{$\rho$: \textbf{0.1790 $\pm$ 0.0028} \\ Top-1: \textbf{0.2764 $\pm$ 0.0051}} & \shortstack{$\rho$: \textbf{0.1567 $\pm$ 0.0145} \\ Top-1: \textbf{0.2743 $\pm$ 0.0052}} & \shortstack{$\rho$: \textbf{0.1538 $\pm$ 0.0153} \\ Top-1: \textbf{0.2732 $\pm$ 0.0023}} \\
 & 7B & \shortstack{$\rho$: \textbf{0.4911 $\pm$ 0.0043} \\ Top-1: 0.2894 $\pm$ 0.0067} & \shortstack{$\rho$: \textbf{0.4956 $\pm$ 0.0037} \\ Top-1: 0.2981 $\pm$ 0.0069} & \shortstack{$\rho$: \underline{0.4838 $\pm$ 0.0016} \\ Top-1: \underline{0.2997 $\pm$ 0.0036}} & \shortstack{$\rho$: \underline{0.4827 $\pm$ 0.0018} \\ Top-1: \underline{0.2976 $\pm$ 0.0045}} \\
\bottomrule
\end{tabular}%
}
\caption{Model-scaling results on the test split. Each cell reports Spearman $\rho$ and Top-1 accuracy as mean $\pm$ sample standard deviation across five seeds. Baselines are single deterministic evaluations and therefore have zero reported standard deviation. Bold and underlined values are respectively best and second-best among methods at the same model size and $k$.}
\label{tab:scaling-combined-test}
\end{table*}


==> scaling_table_across_methods_disp.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Method & Model & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
\multirow{3}{*}{Baseline} & 0.5B & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0285 $\pm$ 0.0000 \\ Top-1: 0.2119 $\pm$ 0.0000} \\
 & 1.5B & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0419 $\pm$ 0.0000 \\ Top-1: 0.1845 $\pm$ 0.0000} \\
 & 7B & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4508 $\pm$ 0.0000 \\ Top-1: 0.2913 $\pm$ 0.0000} \\
\midrule
\multirow{3}{*}{Mallows-RCPO} & 0.5B & \shortstack{$\rho$: 0.1677 $\pm$ 0.0053 \\ Top-1: \textbf{0.2899 $\pm$ 0.0026}} & \shortstack{$\rho$: 0.1660 $\pm$ 0.0048 \\ Top-1: \textbf{0.2886 $\pm$ 0.0029}} & \shortstack{$\rho$: 0.1666 $\pm$ 0.0055 \\ Top-1: \textbf{0.2898 $\pm$ 0.0037}} & \shortstack{$\rho$: 0.1658 $\pm$ 0.0067 \\ Top-1: \textbf{0.2886 $\pm$ 0.0035}} \\
 & 1.5B & \shortstack{$\rho$: 0.0668 $\pm$ 0.0117 \\ Top-1: 0.2485 $\pm$ 0.0018} & \shortstack{$\rho$: 0.0711 $\pm$ 0.0132 \\ Top-1: 0.2488 $\pm$ 0.0017} & \shortstack{$\rho$: 0.0626 $\pm$ 0.0054 \\ Top-1: 0.2481 $\pm$ 0.0013} & \shortstack{$\rho$: 0.0606 $\pm$ 0.0060 \\ Top-1: 0.2469 $\pm$ 0.0039} \\
 & 7B & \shortstack{$\rho$: 0.5129 $\pm$ 0.0029 \\ Top-1: \textbf{0.3348 $\pm$ 0.0041}} & \shortstack{$\rho$: 0.5123 $\pm$ 0.0019 \\ Top-1: \textbf{0.3360 $\pm$ 0.0031}} & \shortstack{$\rho$: \underline{0.5115 $\pm$ 0.0034} \\ Top-1: \textbf{0.3359 $\pm$ 0.0034}} & \shortstack{$\rho$: \underline{0.5117 $\pm$ 0.0051} \\ Top-1: \textbf{0.3364 $\pm$ 0.0051}} \\
\midrule
\multirow{3}{*}{PL-DPO} & 0.5B & \shortstack{$\rho$: 0.1319 $\pm$ 0.0049 \\ Top-1: 0.2589 $\pm$ 0.0031} & \shortstack{$\rho$: 0.1413 $\pm$ 0.0054 \\ Top-1: 0.2537 $\pm$ 0.0027} & \shortstack{$\rho$: 0.1547 $\pm$ 0.0068 \\ Top-1: 0.2547 $\pm$ 0.0032} & \shortstack{$\rho$: 0.1541 $\pm$ 0.0072 \\ Top-1: 0.2559 $\pm$ 0.0023} \\
 & 1.5B & \shortstack{$\rho$: 0.0412 $\pm$ 0.0035 \\ Top-1: 0.2246 $\pm$ 0.0038} & \shortstack{$\rho$: 0.0582 $\pm$ 0.0047 \\ Top-1: 0.2288 $\pm$ 0.0031} & \shortstack{$\rho$: 0.0748 $\pm$ 0.0056 \\ Top-1: 0.2357 $\pm$ 0.0024} & \shortstack{$\rho$: 0.0729 $\pm$ 0.0083 \\ Top-1: 0.2343 $\pm$ 0.0029} \\
 & 7B & \shortstack{$\rho$: 0.4859 $\pm$ 0.0035 \\ Top-1: \underline{0.3190 $\pm$ 0.0046}} & \shortstack{$\rho$: 0.4909 $\pm$ 0.0023 \\ Top-1: \underline{0.3144 $\pm$ 0.0029}} & \shortstack{$\rho$: 0.4947 $\pm$ 0.0008 \\ Top-1: \underline{0.3155 $\pm$ 0.0041}} & \shortstack{$\rho$: 0.4935 $\pm$ 0.0018 \\ Top-1: \underline{0.3140 $\pm$ 0.0038}} \\
\midrule
\multirow{3}{*}{f-RPO-TV} & 0.5B & \shortstack{$\rho$: \textbf{0.1997 $\pm$ 0.0063} \\ Top-1: \underline{0.2726 $\pm$ 0.0042}} & \shortstack{$\rho$: \underline{0.2086 $\pm$ 0.0052} \\ Top-1: \underline{0.2709 $\pm$ 0.0025}} & \shortstack{$\rho$: \textbf{0.2113 $\pm$ 0.0043} \\ Top-1: \underline{0.2690 $\pm$ 0.0023}} & \shortstack{$\rho$: \textbf{0.2110 $\pm$ 0.0044} \\ Top-1: \underline{0.2693 $\pm$ 0.0018}} \\
 & 1.5B & \shortstack{$\rho$: \underline{0.1369 $\pm$ 0.0098} \\ Top-1: \underline{0.2616 $\pm$ 0.0063}} & \shortstack{$\rho$: \underline{0.1524 $\pm$ 0.0055} \\ Top-1: \underline{0.2638 $\pm$ 0.0048}} & \shortstack{$\rho$: \underline{0.1573 $\pm$ 0.0079} \\ Top-1: \underline{0.2652 $\pm$ 0.0056}} & \shortstack{$\rho$: \underline{0.1618 $\pm$ 0.0064} \\ Top-1: \underline{0.2694 $\pm$ 0.0043}} \\
 & 7B & \shortstack{$\rho$: \textbf{0.5323 $\pm$ 0.0019} \\ Top-1: 0.3075 $\pm$ 0.0019} & \shortstack{$\rho$: \textbf{0.5323 $\pm$ 0.0025} \\ Top-1: 0.3001 $\pm$ 0.0038} & \shortstack{$\rho$: \textbf{0.5302 $\pm$ 0.0014} \\ Top-1: 0.2972 $\pm$ 0.0031} & \shortstack{$\rho$: \textbf{0.5289 $\pm$ 0.0022} \\ Top-1: 0.2962 $\pm$ 0.0022} \\
\midrule
\multirow{3}{*}{f-RPO reverse KL} & 0.5B & \shortstack{$\rho$: \underline{0.1990 $\pm$ 0.0057} \\ Top-1: 0.2677 $\pm$ 0.0017} & \shortstack{$\rho$: \textbf{0.2128 $\pm$ 0.0079} \\ Top-1: 0.2645 $\pm$ 0.0038} & \shortstack{$\rho$: \underline{0.2029 $\pm$ 0.0063} \\ Top-1: 0.2595 $\pm$ 0.0011} & \shortstack{$\rho$: \underline{0.2020 $\pm$ 0.0058} \\ Top-1: 0.2602 $\pm$ 0.0020} \\
 & 1.5B & \shortstack{$\rho$: \textbf{0.1589 $\pm$ 0.0102} \\ Top-1: \textbf{0.2689 $\pm$ 0.0029}} & \shortstack{$\rho$: \textbf{0.1929 $\pm$ 0.0082} \\ Top-1: \textbf{0.2755 $\pm$ 0.0024}} & \shortstack{$\rho$: \textbf{0.1740 $\pm$ 0.0132} \\ Top-1: \textbf{0.2700 $\pm$ 0.0045}} & \shortstack{$\rho$: \textbf{0.1777 $\pm$ 0.0135} \\ Top-1: \textbf{0.2697 $\pm$ 0.0049}} \\
 & 7B & \shortstack{$\rho$: \underline{0.5238 $\pm$ 0.0017} \\ Top-1: 0.3001 $\pm$ 0.0027} & \shortstack{$\rho$: \underline{0.5199 $\pm$ 0.0020} \\ Top-1: 0.2980 $\pm$ 0.0011} & \shortstack{$\rho$: 0.5108 $\pm$ 0.0015 \\ Top-1: 0.2977 $\pm$ 0.0019} & \shortstack{$\rho$: 0.5097 $\pm$ 0.0019 \\ Top-1: 0.2976 $\pm$ 0.0016} \\
\bottomrule
\end{tabular}%
}
\caption{Model-scaling results on the train split. Each cell reports Spearman $\rho$ and Top-1 accuracy as mean $\pm$ sample standard deviation across five seeds. Baselines are single deterministic evaluations and therefore have zero reported standard deviation. Bold and underlined values are respectively best and second-best among methods at the same model size and $k$. (With Dispersion)}
\label{tab:scaling-combined-train}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Method & Model & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
\multirow{3}{*}{Baseline} & 0.5B & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} & \shortstack{$\rho$: 0.0314 $\pm$ 0.0000 \\ Top-1: 0.2385 $\pm$ 0.0000} \\
 & 1.5B & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} & \shortstack{$\rho$: -0.0431 $\pm$ 0.0000 \\ Top-1: 0.2033 $\pm$ 0.0000} \\
 & 7B & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: \underline{0.2927 $\pm$ 0.0000}} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} & \shortstack{$\rho$: 0.4390 $\pm$ 0.0000 \\ Top-1: 0.2927 $\pm$ 0.0000} \\
\midrule
\multirow{3}{*}{Mallows-RCPO} & 0.5B & \shortstack{$\rho$: 0.1309 $\pm$ 0.0040 \\ Top-1: \underline{0.2829 $\pm$ 0.0062}} & \shortstack{$\rho$: 0.1319 $\pm$ 0.0067 \\ Top-1: \underline{0.2856 $\pm$ 0.0056}} & \shortstack{$\rho$: 0.1294 $\pm$ 0.0063 \\ Top-1: \underline{0.2829 $\pm$ 0.0056}} & \shortstack{$\rho$: 0.1309 $\pm$ 0.0047 \\ Top-1: \underline{0.2835 $\pm$ 0.0068}} \\
 & 1.5B & \shortstack{$\rho$: 0.0431 $\pm$ 0.0229 \\ Top-1: 0.2428 $\pm$ 0.0083} & \shortstack{$\rho$: 0.0491 $\pm$ 0.0253 \\ Top-1: 0.2450 $\pm$ 0.0118} & \shortstack{$\rho$: 0.0319 $\pm$ 0.0063 \\ Top-1: 0.2352 $\pm$ 0.0080} & \shortstack{$\rho$: 0.0311 $\pm$ 0.0060 \\ Top-1: 0.2358 $\pm$ 0.0061} \\
 & 7B & \shortstack{$\rho$: 0.4682 $\pm$ 0.0042 \\ Top-1: \textbf{0.3003 $\pm$ 0.0067}} & \shortstack{$\rho$: 0.4671 $\pm$ 0.0038 \\ Top-1: \underline{0.3024 $\pm$ 0.0049}} & \shortstack{$\rho$: 0.4659 $\pm$ 0.0040 \\ Top-1: \underline{0.2997 $\pm$ 0.0068}} & \shortstack{$\rho$: 0.4693 $\pm$ 0.0043 \\ Top-1: \underline{0.3019 $\pm$ 0.0045}} \\
\midrule
\multirow{3}{*}{PL-DPO} & 0.5B & \shortstack{$\rho$: 0.0980 $\pm$ 0.0055 \\ Top-1: 0.2780 $\pm$ 0.0041} & \shortstack{$\rho$: 0.1035 $\pm$ 0.0058 \\ Top-1: 0.2775 $\pm$ 0.0036} & \shortstack{$\rho$: 0.1143 $\pm$ 0.0046 \\ Top-1: 0.2808 $\pm$ 0.0041} & \shortstack{$\rho$: 0.1108 $\pm$ 0.0051 \\ Top-1: 0.2813 $\pm$ 0.0023} \\
 & 1.5B & \shortstack{$\rho$: 0.0098 $\pm$ 0.0062 \\ Top-1: 0.2287 $\pm$ 0.0049} & \shortstack{$\rho$: 0.0276 $\pm$ 0.0061 \\ Top-1: 0.2341 $\pm$ 0.0065} & \shortstack{$\rho$: 0.0434 $\pm$ 0.0028 \\ Top-1: 0.2428 $\pm$ 0.0049} & \shortstack{$\rho$: 0.0433 $\pm$ 0.0052 \\ Top-1: 0.2407 $\pm$ 0.0040} \\
 & 7B & \shortstack{$\rho$: 0.4458 $\pm$ 0.0035 \\ Top-1: \textbf{0.3003 $\pm$ 0.0012}} & \shortstack{$\rho$: 0.4466 $\pm$ 0.0040 \\ Top-1: \textbf{0.3041 $\pm$ 0.0065}} & \shortstack{$\rho$: 0.4517 $\pm$ 0.0018 \\ Top-1: \textbf{0.3046 $\pm$ 0.0031}} & \shortstack{$\rho$: 0.4522 $\pm$ 0.0029 \\ Top-1: \textbf{0.3062 $\pm$ 0.0019}} \\
\midrule
\multirow{3}{*}{f-RPO-TV} & 0.5B & \shortstack{$\rho$: \underline{0.1410 $\pm$ 0.0080} \\ Top-1: 0.2797 $\pm$ 0.0045} & \shortstack{$\rho$: \underline{0.1481 $\pm$ 0.0044} \\ Top-1: 0.2786 $\pm$ 0.0056} & \shortstack{$\rho$: \underline{0.1507 $\pm$ 0.0067} \\ Top-1: 0.2791 $\pm$ 0.0051} & \shortstack{$\rho$: \underline{0.1481 $\pm$ 0.0048} \\ Top-1: 0.2791 $\pm$ 0.0033} \\
 & 1.5B & \shortstack{$\rho$: \underline{0.1063 $\pm$ 0.0094} \\ Top-1: \underline{0.2602 $\pm$ 0.0079}} & \shortstack{$\rho$: \underline{0.1222 $\pm$ 0.0072} \\ Top-1: \underline{0.2645 $\pm$ 0.0049}} & \shortstack{$\rho$: \underline{0.1287 $\pm$ 0.0073} \\ Top-1: \underline{0.2667 $\pm$ 0.0059}} & \shortstack{$\rho$: \underline{0.1338 $\pm$ 0.0054} \\ Top-1: \underline{0.2710 $\pm$ 0.0019}} \\
 & 7B & \shortstack{$\rho$: \underline{0.4856 $\pm$ 0.0015} \\ Top-1: 0.2856 $\pm$ 0.0024} & \shortstack{$\rho$: \underline{0.4864 $\pm$ 0.0036} \\ Top-1: 0.2856 $\pm$ 0.0015} & \shortstack{$\rho$: \textbf{0.4856 $\pm$ 0.0030} \\ Top-1: 0.2813 $\pm$ 0.0035} & \shortstack{$\rho$: \textbf{0.4851 $\pm$ 0.0024} \\ Top-1: 0.2808 $\pm$ 0.0031} \\
\midrule
\multirow{3}{*}{f-RPO reverse KL} & 0.5B & \shortstack{$\rho$: \textbf{0.1601 $\pm$ 0.0101} \\ Top-1: \textbf{0.2894 $\pm$ 0.0078}} & \shortstack{$\rho$: \textbf{0.1769 $\pm$ 0.0075} \\ Top-1: \textbf{0.2932 $\pm$ 0.0062}} & \shortstack{$\rho$: \textbf{0.1677 $\pm$ 0.0077} \\ Top-1: \textbf{0.2911 $\pm$ 0.0049}} & \shortstack{$\rho$: \textbf{0.1682 $\pm$ 0.0080} \\ Top-1: \textbf{0.2894 $\pm$ 0.0040}} \\
 & 1.5B & \shortstack{$\rho$: \textbf{0.1336 $\pm$ 0.0116} \\ Top-1: \textbf{0.2748 $\pm$ 0.0045}} & \shortstack{$\rho$: \textbf{0.1703 $\pm$ 0.0106} \\ Top-1: \textbf{0.2791 $\pm$ 0.0051}} & \shortstack{$\rho$: \textbf{0.1524 $\pm$ 0.0123} \\ Top-1: \textbf{0.2775 $\pm$ 0.0031}} & \shortstack{$\rho$: \textbf{0.1583 $\pm$ 0.0129} \\ Top-1: \textbf{0.2780 $\pm$ 0.0053}} \\
 & 7B & \shortstack{$\rho$: \textbf{0.4909 $\pm$ 0.0032} \\ Top-1: 0.2889 $\pm$ 0.0059} & \shortstack{$\rho$: \textbf{0.4940 $\pm$ 0.0020} \\ Top-1: 0.2976 $\pm$ 0.0093} & \shortstack{$\rho$: \underline{0.4831 $\pm$ 0.0030} \\ Top-1: 0.2986 $\pm$ 0.0035} & \shortstack{$\rho$: \underline{0.4817 $\pm$ 0.0016} \\ Top-1: 0.3003 $\pm$ 0.0030} \\
\bottomrule
\end{tabular}%
}
\caption{Model-scaling results on the test split. Each cell reports Spearman $\rho$ and Top-1 accuracy as mean $\pm$ sample standard deviation across five seeds. Baselines are single deterministic evaluations and therefore have zero reported standard deviation. Bold and underlined values are respectively best and second-best among methods at the same model size and $k$. (With dispersion)}
\label{tab:scaling-combined-test}
\end{table*}


==> shorthand.tex <==
\usepackage{xfrac}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage{tabularray}
% \usepackage{environ}         % provides \BODY
% \usepackage{etoolbox}        % provides \ifdimcomp
% \usepackage{graphicx}        % provides \resizebox

% \newlength{\myl}
% \let\origequation=\equation
% \let\origendequation=\endequation

% \RenewEnviron{equation}{
%   \settowidth{\myl}{$\BODY$}                       % calculate width and save as \myl
%   \origequation
%   \ifdimcomp{\the\linewidth}{>}{\the\myl}
%   {\ensuremath{\BODY}}                             % True
%   {\resizebox{\linewidth}{!}{\ensuremath{\BODY}}}  % False
%   \origendequation
% }

\newcommand*{\myDots}{\ifmmode\mathellipsis\else.\kern-0.13em.\kern-0.13em.\fi} % touching at \kern-0.1725em

\usepackage{hyperref} % ensure this is in your preamble

\newcommand{\sref}[1]{\hyperref[#1]{§\ref*{#1}}}

\newcommand{\on}[1]{#1_{\shortparallel}}
\newcommand{\off}[1]{#1_{\perp}}
\newcommand{\flt}[1]{#1_{\vdash}}
\newcommand{\bld}[1]{\mathbf{#1}}
\newcommand{\xt}{\Tilde{x}}
\newcommand{\wt}{\Tilde{w}}
\newcommand{\At}{\Tilde{\bld{A}}}
\newcommand{\at}{\Tilde{a}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\bXt}{\Tilde{\mathbf{X}}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbbm{E}}
\newcommand{\inner}[2]{ #1\odot #2}
\newcommand{\Inner}[2]{ \langle #1 \; , \; #2 \rangle}
\newcommand{\iter}[2]{ #1^{(#2)}}
\DeclareMathOperator{\vect}{vec}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bxt}{\Tilde{\bx}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bh}{\mathbf{h}}

\newcommand{\bM}{\mathbf{M}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bL}{\mathbf{L}}
%\newcommand{\bh}{{\mathbb H}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bmut}{\Tilde{\bmu}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bxit}{\Tilde{\bxi}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\ex}{\epsilon_x}
\newcommand{\exi}{\epsilon_{\xi}}
\newcommand{\exxi}{\epsilon_{x \xi}}

\newcommand{\co}{{\cal O}}
\newcommand{\ca}{{\cal A}}
\newcommand{\cb}{{\cal B}}
\newcommand{\cd}{{\cal D}}
\newcommand{\cdb}{{\cal D}^{\rm b}}
\newcommand{\cc}{{\cal C}}
\newcommand{\ck}{{\cal K}}
\newcommand{\cq}{{\cal Q}}
\newcommand{\ce}{{\cal E}}
\newcommand{\ct}{{\cal T}}
\newcommand{\cg}{{\cal G}}
\newcommand{\ch}{{\cal H}}
\newcommand{\cm}{{\cal M}}
\newcommand{\ci}{{\cal I}}
\newcommand{\cj}{{\cal J}}
\newcommand{\cw}{{\cal W}}
\newcommand{\cl}{{\cal L}}
\newcommand{\cf}{{\cal F}}
\newcommand{\cv}{{\cal V}}
\newcommand{\cp}{{\cal P}}
\newcommand{\cu}{{\cal U}}
\newcommand{\cx}{{\cal X}}
\newcommand{\cy}{{\cal Y}}
\newcommand{\cz}{{\cal Z}}
\newcommand{\cs}{{\cal S}}
\newcommand{\cn}{{\cal N}}
\newcommand{\calr}{{\cal R}}

\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\cluster}{cluster}


\newcommand{\bbs}{{\mathbb S}}
\newcommand{\reals}{{\mathbb R}}
\newcommand{\nat}{{\mathbb N}}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\complex}{{\mathbb C}}
%\newcommand{\zero}{{\vec 0}}
\newcommand{\zero}{{\mathbf{0}}}
\newcommand{\ndist}{\mathsf{N}}
\newcommand{\Dclust}{{\mathcal{D}_{\text{clusters}}}}



%\newcommand{\E}[1]{\mbox{E}\left[#1\right] }
%\newcommand{\prob}[1]{{\rm Prob}\left\{ #1 \right\} }

%\newcommand{\proofbox}{\begin{flushright}$\Box$\end{flushright}}
\newcommand{\proofbox}{\hfill $\Box$}

\newcommand{\commentjf}[1]{{\bf [#1]}}

\newcommand{\diag}{\mathrm{diag}}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\V}{\mathbb{V}}
\DeclareMathOperator{\bin}{bin}
\DeclareMathOperator{\betadist}{Beta}


\newcommand{\unifdist}[2]{\cu(#1,#2)}

%\newcommand{\D}{\mathcal{D}}
\newcommand{\tn}{{\tilde{n}}}
%\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\binner}[1]{\biggl< #1 \biggr>}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\snorm}[1]{\|#1\|} %small norm
\newcommand{\tbx}{{\tilde{\bx}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\rmax}{R_{\text{max}}}
\newcommand{\rmin}{R_{\text{min}}}

\newcommand{\pref}{\pi_{\rm ref}}
\newcommand{\ppol}{\pi_{\theta}}
\newcommand{\pold}{\pi_{\theta_{\rm old}}}
\newcommand{\pluspol}{\pi^+_{\theta_\text{old}}}
\newcommand{\negpol}{\pi^-_{\theta_\text{old}}}
\newcommand{\ppolo}{\pi_{\theta^*}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\gdiv}{\mathbb{D}\infdivx}
\newcommand{\kldiv}{\mathbb{D}_{\text{KL}}\infdivx}
\newcommand{\fdiv}{\mathbb{D}_{f}\infdivx}
\newcommand{\tvdiv}{\mathbb{D}_{\text{TV}}\infdivx}
\newcommand{\jsdiv}{\mathbb{D}_{\text{JS}}\infdivx}
\newcommand{\dpodiv}{\mathbb{D}_{\text{DPO}}\infdivx}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\effdom}{ED}
\DeclareMathOperator{\clip}{Clip}
\DeclareMathOperator{\Cov}{Cov}

\setlength{\textfloatsep}{8pt} % Adjust to your preference
\newcommand{\Fon}[2]{\E_x\E_{y\sim\pold}\!\left[#1\right]}
\DeclareMathOperator{\SoftMax}{SoftMax}




==> tables/main_qualitative_gen_eg.tex <==
% Requires: booktabs, tabularx, xcolor[table]
\begin{table}[!ht]
\centering
\caption{
Qualitative example from Qwen2.5-1.5B on AlpacaEval.
For the prompt \emph{``Is queue an ADT or a data structure?''},
both prior ranked-alignment methods degenerate, whereas both
$f$-RPO variants give coherent answers identifying a queue as an
abstract data type with concrete data-structure implementations.
Judge denotes the GPT-4.1-mini preference against the unaligned
base model ($2$: aligned model preferred; $1$: base preferred).
}
\label{tab:qualitative-main}
\scriptsize
\setlength{\tabcolsep}{3pt}

\begin{tabularx}{\columnwidth}{l c X}
\toprule
Method & Judge & Generation excerpt \\
\midrule

PL-DPO
& 1
& Repeats ``1.1.1.1\ldots'' instead of answering. \\

Mallows-RCPO
& 1
& Repeats the prompt interleaved with nonsensical tokens. \\

\rowcolor{gray!10}
$f$-RPO-RKL
& \textbf{2}
& ``An ADT is a high-level abstraction that defines a set of
operations \ldots'' It explains that a queue is an ADT that can be
implemented using arrays or linked structures. \\

\rowcolor{gray!10}
$f$-RPO-TV
& \textbf{2}
& Explains FIFO behavior and operations such as
\texttt{enqueue} and \texttt{dequeue}, distinguishing the queue
abstraction from its concrete implementation. \\

\bottomrule
\end{tabularx}
\end{table}

==> tables/tab_dispersion.tex <==
% Requires: booktabs, multirow
% Values are mean +- SEM; source screenshots reported sample SD over five seeds.
\begin{table}[t]
\centering
\caption{Prompt-dependent dispersion ablation at $k=5$. Spearman $\rho$ is reported as mean $\pm$ SEM over five seeds.}
\label{tab:dispersion-ablation}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcc}
\toprule
Model & Divergence & Without $\phi(x)$ & With $\phi(x)$ \\
\midrule
\multirow{2}{*}{Qwen 0.5B}
 & TV  & $0.1492 \pm 0.0017$ & $0.1481 \pm 0.0021$ \\
 & RKL & $0.1648 \pm 0.0039$ & $\mathbf{0.1682 \pm 0.0036}$ \\
\midrule
\multirow{2}{*}{Qwen 1.5B}
 & TV  & $0.1288 \pm 0.0035$ & $0.1338 \pm 0.0024$ \\
 & RKL & $0.1538 \pm 0.0068$ & $\mathbf{0.1583 \pm 0.0058}$ \\
\midrule
\multirow{2}{*}{Qwen 7B}
 & TV  & $\mathbf{0.4858 \pm 0.0005}$ & $0.4851 \pm 0.0011$ \\
 & RKL & $\mathbf{0.4827 \pm 0.0008}$ & $0.4817 \pm 0.0007$ \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/tab_divergence_replication_placeholder.tex <==
% Focused future experiment: one additional family, k=5 only.
% Do not include in the submitted paper until all cells are populated.
\begin{table}[t]
\centering
\caption{Planned cross-family replication of the divergence comparison on Llama 3.2 3B at $k=5$. Values will be mean $\pm$ SEM over five seeds.}
\label{tab:divergence-replication}
\small
\begin{tabular}{lcc}
\toprule
Divergence & Spearman $\rho$ & Top-1 \\
\midrule
KL                & -- & -- \\
Reverse KL        & -- & -- \\
Pearson $\chi^2$  & -- & -- \\
Squared Hellinger & -- & -- \\
Jensen--Shannon   & -- & -- \\
Total variation   & -- & -- \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/divergence_compare_full_v0.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\multicolumn{8}{c}{\textit{Ranking performance}} \\
\midrule
Divergence & Spearman $\rho$ & Kendall $\tau$ & Pairwise acc. & Top-1 acc. & Exact match & MAE & RMSE \\
\midrule
Base model (Qwen2.5-0.5B) & 0.0285 & 0.0277 & 0.5139 & 0.2119 & 0.0125 & 1.5599 & 1.8767 \\
KL & 0.1304 $\pm$ 0.0021 & 0.1098 $\pm$ 0.0020 & 0.5549 $\pm$ 0.0010 & 0.2438 $\pm$ 0.0009 & 0.0165 $\pm$ 0.0007 & 1.4516 $\pm$ 0.0026 & 1.7577 $\pm$ 0.0030 \\
Reverse KL & 0.2027 $\pm$ 0.0031 & 0.1670 $\pm$ 0.0026 & 0.5835 $\pm$ 0.0013 & 0.2607 $\pm$ 0.0003 & 0.0173 $\pm$ 0.0004 & 1.3755 $\pm$ 0.0031 & 1.6748 $\pm$ 0.0039 \\
Pearson $\chi^2$ & 0.1541 $\pm$ 0.0013 & 0.1292 $\pm$ 0.0010 & 0.5646 $\pm$ 0.0005 & 0.2542 $\pm$ 0.0009 & 0.0173 $\pm$ 0.0005 & 1.4244 $\pm$ 0.0016 & 1.7289 $\pm$ 0.0019 \\
Squared Hellinger & 0.1288 $\pm$ 0.0008 & 0.1077 $\pm$ 0.0006 & 0.5538 $\pm$ 0.0003 & 0.2472 $\pm$ 0.0008 & 0.0130 $\pm$ 0.0005 & 1.4539 $\pm$ 0.0007 & 1.7608 $\pm$ 0.0009 \\
Jensen--Shannon & 0.1471 $\pm$ 0.0015 & 0.1227 $\pm$ 0.0012 & 0.5613 $\pm$ 0.0006 & 0.2536 $\pm$ 0.0015 & 0.0159 $\pm$ 0.0004 & 1.4325 $\pm$ 0.0019 & 1.7379 $\pm$ 0.0021 \\
Total variation & 0.2128 $\pm$ 0.0014 & 0.1750 $\pm$ 0.0012 & 0.5875 $\pm$ 0.0006 & 0.2694 $\pm$ 0.0012 & 0.0187 $\pm$ 0.0002 & 1.3609 $\pm$ 0.0015 & 1.6603 $\pm$ 0.0019 \\
\bottomrule
\end{tabular}%
}
\vspace{0.5em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textit{Candidate-score distribution}} \\
\midrule
Divergence & Entropy & Norm. entropy & Effective count \\
\midrule
Base model (Qwen2.5-0.5B) & 1.5501 & 0.9631 & 4.7421 \\
KL & 1.5455 $\pm$ 0.0001 & 0.9603 $\pm$ 0.0001 & 4.7237 $\pm$ 0.0003 \\
Reverse KL & 1.5430 $\pm$ 0.0002 & 0.9587 $\pm$ 0.0001 & 4.7125 $\pm$ 0.0008 \\
Pearson $\chi^2$ & 1.5442 $\pm$ 0.0001 & 0.9594 $\pm$ 0.0001 & 4.7188 $\pm$ 0.0003 \\
Squared Hellinger & 1.5445 $\pm$ 0.0001 & 0.9596 $\pm$ 0.0001 & 4.7196 $\pm$ 0.0004 \\
Jensen--Shannon & 1.5449 $\pm$ 0.0001 & 0.9599 $\pm$ 0.0000 & 4.7210 $\pm$ 0.0003 \\
Total variation & 1.5405 $\pm$ 0.0002 & 0.9572 $\pm$ 0.0001 & 4.7050 $\pm$ 0.0008 \\
\bottomrule
\end{tabular}%
}
\caption{Effect of the $f$-divergence on staged f-RPO at $k=5$ on the train split. The base-model row is a single deterministic evaluation. For aligned models, entries report the mean $\pm$ standard error over five seeds, where $\mathrm{SE}=s/\sqrt{5}$ and $s$ is the sample standard deviation across seeds.}
\label{tab:frpo-divergence-k5-all-train}
\end{table*}

\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\multicolumn{8}{c}{\textit{Ranking performance}} \\
\midrule
Divergence & Spearman $\rho$ & Kendall $\tau$ & Pairwise acc. & Top-1 acc. & Exact match & MAE & RMSE \\
\midrule
Base model (Qwen2.5-0.5B) & 0.0314 & 0.0320 & 0.5160 & 0.2385 & 0.0244 & 1.5631 & 1.8644 \\
KL & 0.0928 $\pm$ 0.0019 & 0.0796 $\pm$ 0.0017 & 0.5398 $\pm$ 0.0008 & 0.2694 $\pm$ 0.0029 & 0.0298 $\pm$ 0.0000 & 1.4955 $\pm$ 0.0021 & 1.7899 $\pm$ 0.0019 \\
Reverse KL & 0.1648 $\pm$ 0.0039 & 0.1340 $\pm$ 0.0031 & 0.5670 $\pm$ 0.0016 & 0.2894 $\pm$ 0.0010 & 0.0320 $\pm$ 0.0005 & 1.4131 $\pm$ 0.0053 & 1.7066 $\pm$ 0.0048 \\
Pearson $\chi^2$ & 0.1048 $\pm$ 0.0012 & 0.0879 $\pm$ 0.0010 & 0.5440 $\pm$ 0.0005 & 0.2770 $\pm$ 0.0026 & 0.0304 $\pm$ 0.0010 & 1.4784 $\pm$ 0.0020 & 1.7749 $\pm$ 0.0019 \\
Squared Hellinger & 0.0937 $\pm$ 0.0005 & 0.0792 $\pm$ 0.0006 & 0.5396 $\pm$ 0.0003 & 0.2808 $\pm$ 0.0007 & 0.0314 $\pm$ 0.0018 & 1.4862 $\pm$ 0.0011 & 1.7861 $\pm$ 0.0015 \\
Jensen--Shannon & 0.1044 $\pm$ 0.0010 & 0.0881 $\pm$ 0.0011 & 0.5441 $\pm$ 0.0005 & 0.2797 $\pm$ 0.0016 & 0.0314 $\pm$ 0.0011 & 1.4782 $\pm$ 0.0012 & 1.7745 $\pm$ 0.0013 \\
Total variation & 0.1492 $\pm$ 0.0017 & 0.1233 $\pm$ 0.0016 & 0.5616 $\pm$ 0.0008 & 0.2780 $\pm$ 0.0018 & 0.0309 $\pm$ 0.0007 & 1.4333 $\pm$ 0.0019 & 1.7252 $\pm$ 0.0020 \\
\bottomrule
\end{tabular}%
}
\vspace{0.5em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textit{Candidate-score distribution}} \\
\midrule
Divergence & Entropy & Norm. entropy & Effective count \\
\midrule
Base model (Qwen2.5-0.5B) & 1.5474 & 0.9614 & 4.7278 \\
KL & 1.5433 $\pm$ 0.0001 & 0.9589 $\pm$ 0.0001 & 4.7133 $\pm$ 0.0003 \\
Reverse KL & 1.5413 $\pm$ 0.0001 & 0.9577 $\pm$ 0.0001 & 4.7043 $\pm$ 0.0004 \\
Pearson $\chi^2$ & 1.5422 $\pm$ 0.0001 & 0.9582 $\pm$ 0.0001 & 4.7086 $\pm$ 0.0004 \\
Squared Hellinger & 1.5424 $\pm$ 0.0001 & 0.9583 $\pm$ 0.0001 & 4.7087 $\pm$ 0.0005 \\
Jensen--Shannon & 1.5428 $\pm$ 0.0001 & 0.9586 $\pm$ 0.0001 & 4.7105 $\pm$ 0.0004 \\
Total variation & 1.5387 $\pm$ 0.0003 & 0.9560 $\pm$ 0.0002 & 4.6955 $\pm$ 0.0010 \\
\bottomrule
\end{tabular}%
}
\caption{Effect of the $f$-divergence on staged f-RPO at $k=5$ on the test split. The base-model row is a single deterministic evaluation. For aligned models, entries report the mean $\pm$ standard error over five seeds, where $\mathrm{SE}=s/\sqrt{5}$ and $s$ is the sample standard deviation across seeds.}
\label{tab:frpo-divergence-k5-all-test}
\end{table*}


==> tabs/fdiv_mallows.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Aggregate ranking evaluation metrics for Mallows f-divergence RCPO across 5 seed runs. Each cell reports mean (standard deviation).}
\label{tab:mallows_fdiv_seed_aggregate_eval}
\begin{tabular}{lcc}
\toprule
Metric & $\mathrm{Mallows\text{-}FDIV}$ & $\mathrm{Mallows\text{-}FDIV}_{\mathrm{disp}}$ \\
\midrule
Spearman $\rho$ & $-0.1859$ $(0.0018)$ & $-0.1842$ $(0.0012)$ \\
Kendall $\tau$ & $-0.1716$ $(0.0017)$ & $-0.1700$ $(0.0011)$ \\
Rank MAE & $0.9211$ $(0.0008)$ & $0.9203$ $(0.0006)$ \\
Rank RMSE & $1.0326$ $(0.0010)$ & $1.0316$ $(0.0006)$ \\
Pairwise accuracy & $0.4142$ $(0.0009)$ & $0.4150$ $(0.0006)$ \\
Top-1 accuracy & $0.2832$ $(0.0011)$ & $0.2843$ $(0.0011)$ \\
Top-1 in top-$k$ & $0.6576$ $(0.0011)$ & $0.6587$ $(0.0008)$ \\
Exact match rate & $0.2108$ $(0.0008)$ & $0.2111$ $(0.0005)$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/formula_fdiv.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Closed forms for the two-sided variational f-divergence comparison objective used by the Mallows-style f-divergence trainer. Let $v=s_{\mathrm{good}}-s_{\mathrm{bad}}$ and $C_f(v)=g(v)-f^*(g(-v))$. The training loss is $-C_f(v)$.}
\label{tab:fdiv_variational_comparison_forms}
\begin{tabular}{lcccc}
\toprule
Divergence & $g(t)$ & $f^*(g(t))$ & $f^*(g(-v))$ & $C_f(v)=g(v)-f^*(g(-v))$ \\
\midrule
KL & $t$ & $e^{t-1}$ & $e^{-v-1}$ & $v-e^{-v-1}$ \\
Reverse KL & $-e^{-t}$ & $t-1$ & $-v-1$ & $v+1-e^{-v}$ \\
Pearson $\chi^2$ & $t$ & $\frac{1}{4}t^2+t$ & $\frac{1}{4}v^2-v$ & $2v-\frac{1}{4}v^2$ \\
Hellinger & $1-e^{-t}$ & $e^t-1$ & $e^{-v}-1$ & $2-2e^{-v}$ \\
Jensen--Shannon & $\log\sigma(t)$ & $\operatorname{softplus}(t)$ & $\operatorname{softplus}(-v)$ & $-2\operatorname{softplus}(-v)$ \\
Total variation & $\frac{1}{2}\sigma(t)$ & $\frac{1}{2}\sigma(t)$ & $\frac{1}{2}\sigma(-v)$ & $\frac{1}{2}\tanh(v/2)$ \\
\bottomrule
\end{tabular}
\end{table*}


==> tabs/frpo_unnorm_legacyTV.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Aggregate ranking evaluation metrics for FRPO Mallows-style and legacy total-variation FRPO across 5 seed runs. Each cell reports mean (standard deviation).}
\label{tab:new_frpo_mallows_totalvar_seed_aggregate_eval}
\begin{tabular}{lccc}
\toprule
Metric & $\mathrm{FRPO\text{-}Mallows}_{\scriptscriptstyle \mathrm{JS}}$ & $\mathrm{FRPO\text{-}Mallows}_{\scriptscriptstyle \mathrm{JS,disp}}$ & $\mathrm{Legacy\text{-}FRPO}_{\scriptscriptstyle \mathrm{TV}}$ \\
\midrule
Spearman $\rho$ & $-0.1892$ $(0.0024)$ & $-0.1875$ $(0.0014)$ & $-0.1574$ $(0.0032)$ \\
Kendall $\tau$ & $-0.1752$ $(0.0023)$ & $-0.1737$ $(0.0014)$ & $-0.1444$ $(0.0031)$ \\
Rank MAE & $0.9220$ $(0.0011)$ & $0.9210$ $(0.0005)$ & $0.9049$ $(0.0015)$ \\
Rank RMSE & $1.0337$ $(0.0012)$ & $1.0327$ $(0.0006)$ & $1.0154$ $(0.0017)$ \\
Pairwise accuracy & $0.4124$ $(0.0011)$ & $0.4132$ $(0.0007)$ & $0.4278$ $(0.0016)$ \\
Top-1 accuracy & $0.2802$ $(0.0009)$ & $0.2813$ $(0.0002)$ & $0.2950$ $(0.0020)$ \\
Top-1 in top-$k$ & $0.6581$ $(0.0004)$ & $0.6585$ $(0.0007)$ & $0.6700$ $(0.0018)$ \\
Exact match rate & $0.2093$ $(0.0006)$ & $0.2099$ $(0.0002)$ & $0.2211$ $(0.0012)$ \\
\bottomrule
\end{tabular}
\end{table*}


==> tabs/legacy_comparisons.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Metric & JS & KL & Rev. KL & Pearson & Hellinger & TV \\
\midrule
Exact match & 0.2163 $\pm$ 0.0005 & 0.2145 $\pm$ 0.0008 & 0.2147 $\pm$ 0.0006 & 0.2182 $\pm$ 0.0007 & 0.2122 $\pm$ 0.0010 & 0.2211 $\pm$ 0.0012 \\
Top-1 acc. & 0.2857 $\pm$ 0.0007 & 0.2835 $\pm$ 0.0009 & 0.2841 $\pm$ 0.0006 & 0.2889 $\pm$ 0.0011 & 0.2808 $\pm$ 0.0006 & 0.2950 $\pm$ 0.0020 \\
Top-1 in top-k & 0.6610 $\pm$ 0.0013 & 0.6577 $\pm$ 0.0002 & 0.6615 $\pm$ 0.0008 & 0.6624 $\pm$ 0.0015 & 0.6572 $\pm$ 0.0007 & 0.6700 $\pm$ 0.0018 \\
Pairwise acc. mean & 0.4196 $\pm$ 0.0006 & 0.4166 $\pm$ 0.0009 & 0.4184 $\pm$ 0.0004 & 0.4219 $\pm$ 0.0007 & 0.4147 $\pm$ 0.0006 & 0.4278 $\pm$ 0.0016 \\
Pairwise acc. std & 0.3840 $\pm$ 0.0004 & 0.3840 $\pm$ 0.0003 & 0.3835 $\pm$ 0.0004 & 0.3845 $\pm$ 0.0003 & 0.3834 $\pm$ 0.0004 & 0.3844 $\pm$ 0.0003 \\
Kendall mean & -0.1608 $\pm$ 0.0013 & -0.1668 $\pm$ 0.0018 & -0.1632 $\pm$ 0.0007 & -0.1563 $\pm$ 0.0015 & -0.1707 $\pm$ 0.0012 & -0.1444 $\pm$ 0.0031 \\
Kendall std & 0.7679 $\pm$ 0.0008 & 0.7681 $\pm$ 0.0006 & 0.7670 $\pm$ 0.0007 & 0.7689 $\pm$ 0.0006 & 0.7667 $\pm$ 0.0009 & 0.7687 $\pm$ 0.0007 \\
Spearman mean & -0.1748 $\pm$ 0.0015 & -0.1809 $\pm$ 0.0020 & -0.1773 $\pm$ 0.0008 & -0.1701 $\pm$ 0.0015 & -0.1847 $\pm$ 0.0013 & -0.1574 $\pm$ 0.0032 \\
Spearman std & 0.8020 $\pm$ 0.0006 & 0.8018 $\pm$ 0.0006 & 0.8012 $\pm$ 0.0006 & 0.8031 $\pm$ 0.0005 & 0.8005 $\pm$ 0.0007 & 0.8036 $\pm$ 0.0005 \\
MAE mean & 0.9152 $\pm$ 0.0008 & 0.9181 $\pm$ 0.0010 & 0.9167 $\pm$ 0.0006 & 0.9121 $\pm$ 0.0008 & 0.9210 $\pm$ 0.0007 & 0.9049 $\pm$ 0.0015 \\
MAE std & 0.5924 $\pm$ 0.0002 & 0.5917 $\pm$ 0.0006 & 0.5911 $\pm$ 0.0005 & 0.5929 $\pm$ 0.0006 & 0.5907 $\pm$ 0.0006 & 0.5929 $\pm$ 0.0008 \\
RMSE mean & 1.0273 $\pm$ 0.0007 & 1.0305 $\pm$ 0.0009 & 1.0289 $\pm$ 0.0006 & 1.0236 $\pm$ 0.0010 & 1.0338 $\pm$ 0.0008 & 1.0154 $\pm$ 0.0017 \\
RMSE std & 0.6772 $\pm$ 0.0006 & 0.6766 $\pm$ 0.0007 & 0.6759 $\pm$ 0.0007 & 0.6774 $\pm$ 0.0007 & 0.6756 $\pm$ 0.0007 & 0.6765 $\pm$ 0.0008 \\
\bottomrule
\end{tabular}}
\caption{Legacy FRPO divergence aggregate metrics over seeds 1--5. Cells report mean $\pm$ sample standard deviation.}
\label{tab:legacy-frpo-divergences}
\end{table}

\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Metric & JS & KL & Rev. KL & Pearson & Hellinger & TV \\
\midrule
Exact match & 0.2167 $\pm$ 0.0009 & 0.2149 $\pm$ 0.0005 & 0.2149 $\pm$ 0.0008 & 0.2184 $\pm$ 0.0016 & 0.2127 $\pm$ 0.0009 & 0.2217 $\pm$ 0.0008 \\
Top-1 acc. & 0.2866 $\pm$ 0.0012 & 0.2838 $\pm$ 0.0011 & 0.2845 $\pm$ 0.0013 & 0.2896 $\pm$ 0.0014 & 0.2817 $\pm$ 0.0006 & 0.2965 $\pm$ 0.0012 \\
Top-1 in top-k & 0.6616 $\pm$ 0.0010 & 0.6578 $\pm$ 0.0004 & 0.6618 $\pm$ 0.0010 & 0.6627 $\pm$ 0.0012 & 0.6577 $\pm$ 0.0008 & 0.6709 $\pm$ 0.0012 \\
Pairwise acc. mean & 0.4201 $\pm$ 0.0010 & 0.4173 $\pm$ 0.0010 & 0.4186 $\pm$ 0.0007 & 0.4222 $\pm$ 0.0013 & 0.4152 $\pm$ 0.0007 & 0.4287 $\pm$ 0.0008 \\
Pairwise acc. std & 0.3841 $\pm$ 0.0003 & 0.3841 $\pm$ 0.0002 & 0.3837 $\pm$ 0.0005 & 0.3846 $\pm$ 0.0006 & 0.3836 $\pm$ 0.0003 & 0.3846 $\pm$ 0.0003 \\
Kendall mean & -0.1598 $\pm$ 0.0021 & -0.1655 $\pm$ 0.0020 & -0.1629 $\pm$ 0.0014 & -0.1556 $\pm$ 0.0025 & -0.1696 $\pm$ 0.0014 & -0.1426 $\pm$ 0.0017 \\
Kendall std & 0.7683 $\pm$ 0.0005 & 0.7681 $\pm$ 0.0005 & 0.7673 $\pm$ 0.0009 & 0.7692 $\pm$ 0.0012 & 0.7672 $\pm$ 0.0006 & 0.7692 $\pm$ 0.0005 \\
Spearman mean & -0.1736 $\pm$ 0.0022 & -0.1796 $\pm$ 0.0022 & -0.1768 $\pm$ 0.0018 & -0.1692 $\pm$ 0.0024 & -0.1834 $\pm$ 0.0014 & -0.1552 $\pm$ 0.0017 \\
Spearman std & 0.8024 $\pm$ 0.0005 & 0.8019 $\pm$ 0.0004 & 0.8014 $\pm$ 0.0009 & 0.8034 $\pm$ 0.0010 & 0.8011 $\pm$ 0.0005 & 0.8041 $\pm$ 0.0005 \\
MAE mean & 0.9145 $\pm$ 0.0012 & 0.9175 $\pm$ 0.0011 & 0.9163 $\pm$ 0.0014 & 0.9114 $\pm$ 0.0013 & 0.9201 $\pm$ 0.0006 & 0.9036 $\pm$ 0.0009 \\
MAE std & 0.5927 $\pm$ 0.0006 & 0.5918 $\pm$ 0.0003 & 0.5914 $\pm$ 0.0006 & 0.5930 $\pm$ 0.0012 & 0.5910 $\pm$ 0.0007 & 0.5930 $\pm$ 0.0007 \\
RMSE mean & 1.0265 $\pm$ 0.0013 & 1.0299 $\pm$ 0.0011 & 1.0285 $\pm$ 0.0013 & 1.0230 $\pm$ 0.0016 & 1.0331 $\pm$ 0.0007 & 1.0141 $\pm$ 0.0010 \\
RMSE std & 0.6774 $\pm$ 0.0006 & 0.6768 $\pm$ 0.0004 & 0.6761 $\pm$ 0.0007 & 0.6774 $\pm$ 0.0015 & 0.6760 $\pm$ 0.0007 & 0.6767 $\pm$ 0.0007 \\
\bottomrule
\end{tabular}}
\caption{Legacy FRPO divergence aggregate metrics with dispersion over seeds 1--5. Cells report mean $\pm$ sample standard deviation.}
\label{tab:legacy-frpo-divergences-dispersion}
\end{table}


==> tabs/mallows_tab.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Aggregate ranking evaluation metrics for Mallows-RMJ RCPO across 5 seed runs. Each cell reports mean (standard deviation).}
\label{tab:mallows_seed_aggregate_eval}
\begin{tabular}{lcc}
\toprule
Metric & $\mathrm{Mallows\text{-}RMJ}$ & $\mathrm{Mallows\text{-}RMJ}_{\mathrm{disp}}$ \\
\midrule
Spearman $\rho$ & $-0.1482$ $(0.0044)$ & $-0.1459$ $(0.0029)$ \\
Kendall $\tau$ & $-0.1366$ $(0.0040)$ & $-0.1344$ $(0.0026)$ \\
Rank MAE & $0.8980$ $(0.0028)$ & $0.8961$ $(0.0018)$ \\
Rank RMSE & $1.0065$ $(0.0030)$ & $1.0046$ $(0.0018)$ \\
Pairwise accuracy & $0.4317$ $(0.0020)$ & $0.4328$ $(0.0013)$ \\
Top-1 accuracy & $0.3025$ $(0.0024)$ & $0.3045$ $(0.0018)$ \\
Top-1 in top-$k$ & $0.6758$ $(0.0016)$ & $0.6759$ $(0.0011)$ \\
Exact match rate & $0.2217$ $(0.0012)$ & $0.2233$ $(0.0008)$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/prelim_5sd.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Aggregate ranking evaluation metrics across 5 seed runs. Each cell reports mean (standard deviation).}
\label{tab:seed5_aggregate_eval_extended}
\begin{tabular}{lcccccc}
\toprule
Metric & DPO & $\mathrm{FRPO}_{\mathrm{JS}}$ & $\mathrm{FRPO}^{\rm Lin}_{\mathrm{JS}}$ & Legacy $\rm FRPO^{\rm Lin}_{\rm JS}$ & Legacy $\mathrm{FRPO}^{\rm Unif}_{\mathrm{JS}}$ & PLDPO \\
\midrule
Spearman $\rho$ & $-0.1800$ $(0.0016)$ & $-0.1806$ $(0.0009)$ & $-0.1808$ $(0.0015)$ & $-0.1748$ $(0.0015)$ & $-0.1768$ $(0.0019)$ & $-0.1747$ $(0.0009)$ \\
Kendall $\tau$ & $-0.1662$ $(0.0017)$ & $-0.1666$ $(0.0010)$ & $-0.1671$ $(0.0014)$ & $-0.1608$ $(0.0013)$ & $-0.1626$ $(0.0018)$ & $-0.1610$ $(0.0010)$ \\
Rank MAE & $0.9181$ $(0.0009)$ & $0.9185$ $(0.0003)$ & $0.9183$ $(0.0008)$ & $0.9152$ $(0.0008)$ & $0.9168$ $(0.0006)$ & $0.9150$ $(0.0009)$ \\
Rank RMSE & $1.0298$ $(0.0010)$ & $1.0311$ $(0.0005)$ & $1.0309$ $(0.0008)$ & $1.0273$ $(0.0007)$ & $1.0291$ $(0.0007)$ & $1.0267$ $(0.0008)$ \\
Pairwise accuracy & $0.4169$ $(0.0008)$ & $0.4167$ $(0.0005)$ & $0.4165$ $(0.0007)$ & $0.4196$ $(0.0006)$ & $0.4187$ $(0.0009)$ & $0.4195$ $(0.0005)$ \\
Top-1 accuracy & $0.2833$ $(0.0013)$ & $0.2830$ $(0.0005)$ & $0.2824$ $(0.0009)$ & $0.2857$ $(0.0007)$ & $0.2848$ $(0.0005)$ & $0.2849$ $(0.0010)$ \\
Top-1 in top-$k$ & $0.6622$ $(0.0009)$ & $0.6578$ $(0.0007)$ & $0.6587$ $(0.0007)$ & $0.6610$ $(0.0013)$ & $0.6588$ $(0.0011)$ & $0.6627$ $(0.0012)$ \\
Exact match rate & $0.2123$ $(0.0012)$ & $0.2140$ $(0.0007)$ & $0.2138$ $(0.0004)$ & $0.2163$ $(0.0005)$ & $0.2159$ $(0.0006)$ & $0.2156$ $(0.0010)$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/preliminary_tab.tex <==
% \begin{table}[!ht]
% \centering
% \small
% \caption{Aggregate ranking evaluation metrics across 10 seed runs. Each cell reports mean (standard deviation). Note: we used uniform weighting and linear weighting for FRPO first implementation}
% \label{tab:seed_aggregate_eval}
% \begin{tabular}{lcccc}
% \toprule
% Metric & DPO & $\mathrm{FRPO}_{\mathrm{JS}}$ & Legacy $\mathrm{FRPO}_{\mathrm{JS}}$ & PLDPO \\
% \midrule
% Spearman $\rho$      & $-0.1795$ $(0.0017)$ & $-0.1806$ $(0.0011)$ & $-0.1743$ $(0.0014)$ & $-0.1734$ $(0.0018)$ \\
% Kendall $\tau$       & $-0.1657$ $(0.0018)$ & $-0.1668$ $(0.0011)$ & $-0.1604$ $(0.0013)$ & $-0.1599$ $(0.0017)$ \\
% Rank MAE             & $0.9177$ $(0.0011)$  & $0.9185$ $(0.0008)$  & $0.9148$ $(0.0008)$  & $0.9142$ $(0.0012)$  \\
% Rank RMSE            & $1.0293$ $(0.0013)$  & $1.0312$ $(0.0008)$  & $1.0269$ $(0.0009)$  & $1.0259$ $(0.0011)$  \\
% Pairwise accuracy    & $0.4172$ $(0.0009)$  & $0.4166$ $(0.0005)$  & $0.4198$ $(0.0007)$  & $0.4201$ $(0.0008)$  \\
% Top-1 accuracy       & $0.2835$ $(0.0013)$  & $0.2830$ $(0.0008)$  & $0.2860$ $(0.0008)$  & $0.2856$ $(0.0010)$  \\
% Top-1 in top-$k$     & $0.6623$ $(0.0006)$  & $0.6579$ $(0.0007)$  & $0.6612$ $(0.0011)$  & $0.6630$ $(0.0010)$  \\
% Exact match rate     & $0.2127$ $(0.0013)$  & $0.2137$ $(0.0009)$  & $0.2164$ $(0.0005)$  & $0.2159$ $(0.0011)$  \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Aggregate ranking evaluation metrics across 10 seed runs. Each cell reports mean (standard deviation).}
\label{tab:seed_aggregate_eval_extended}
\begin{tabular}{lcccccc}
\toprule
Metric & DPO & $\mathrm{FRPO}_{\mathrm{JS}}$ & $\mathrm{FRPO}^{\rm Lin}_{\mathrm{JS}}$ & Legacy $\rm FRPO^{\rm Lin}_{\rm JS}$ & Legacy $\mathrm{FRPO}^{\rm Unif}_{\mathrm{JS}}$ & PLDPO \\
\midrule
Spearman $\rho$ & $-0.1795$ $(0.0017)$ & $-0.1806$ $(0.0011)$ & $-0.1806$ $(0.0013)$ & $-0.1743$ $(0.0014)$ & $-0.1770$ $(0.0015)$ & $-0.1734$ $(0.0018)$ \\
Kendall $\tau$ & $-0.1657$ $(0.0018)$ & $-0.1668$ $(0.0011)$ & $-0.1669$ $(0.0012)$ & $-0.1604$ $(0.0013)$ & $-0.1629$ $(0.0014)$ & $-0.1599$ $(0.0017)$ \\
Rank MAE & $0.9177$ $(0.0011)$ & $0.9185$ $(0.0008)$ & $0.9183$ $(0.0007)$ & $0.9148$ $(0.0008)$ & $0.9170$ $(0.0006)$ & $0.9142$ $(0.0012)$ \\
Rank RMSE & $1.0293$ $(0.0013)$ & $1.0312$ $(0.0008)$ & $1.0309$ $(0.0007)$ & $1.0269$ $(0.0009)$ & $1.0294$ $(0.0007)$ & $1.0259$ $(0.0011)$ \\
Pairwise accuracy & $0.4172$ $(0.0009)$ & $0.4166$ $(0.0005)$ & $0.4166$ $(0.0006)$ & $0.4198$ $(0.0007)$ & $0.4186$ $(0.0007)$ & $0.4201$ $(0.0008)$ \\
Top-1 accuracy & $0.2835$ $(0.0013)$ & $0.2830$ $(0.0008)$ & $0.2825$ $(0.0010)$ & $0.2860$ $(0.0008)$ & $0.2843$ $(0.0008)$ & $0.2856$ $(0.0010)$ \\
Top-1 in top-$k$ & $0.6623$ $(0.0006)$ & $0.6579$ $(0.0007)$ & $0.6589$ $(0.0007)$ & $0.6612$ $(0.0011)$ & $0.6587$ $(0.0008)$ & $0.6630$ $(0.0010)$ \\
Exact match rate & $0.2127$ $(0.0013)$ & $0.2137$ $(0.0009)$ & $0.2138$ $(0.0005)$ & $0.2164$ $(0.0005)$ & $0.2156$ $(0.0007)$ & $0.2159$ $(0.0011)$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/tanh_mallows.tex <==
\begin{table*}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Aggregate ranking evaluation metrics for the Mallows total-variation tanh RCPO hypothesis across 5 seed runs. Each cell reports mean (standard deviation).}
\label{tab:mallows_tv_tanh_seed_aggregate_eval}
\begin{tabular}{lcc}
\toprule
Metric & $\mathrm{Mallows\text{-}TV}$ & $\mathrm{Mallows\text{-}TV}_{\mathrm{disp}}$ \\
\midrule
Spearman $\rho$ & $-0.1501$ $(0.0044)$ & $-0.1461$ $(0.0033)$ \\
Kendall $\tau$ & $-0.1381$ $(0.0042)$ & $-0.1347$ $(0.0030)$ \\
Rank MAE & $0.8989$ $(0.0028)$ & $0.8962$ $(0.0024)$ \\
Rank RMSE & $1.0074$ $(0.0029)$ & $1.0049$ $(0.0025)$ \\
Pairwise accuracy & $0.4310$ $(0.0021)$ & $0.4327$ $(0.0015)$ \\
Top-1 accuracy & $0.3014$ $(0.0027)$ & $0.3048$ $(0.0017)$ \\
Top-1 in top-$k$ & $0.6747$ $(0.0022)$ & $0.6753$ $(0.0010)$ \\
Exact match rate & $0.2215$ $(0.0016)$ & $0.2230$ $(0.0015)$ \\
\bottomrule
\end{tabular}
\end{table*}

==> test_fdiv_method_topk_tables.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Divergence & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
KL & 0.0851 $\pm$ 0.0050 & 0.0913 $\pm$ 0.0042 & 0.0939 $\pm$ 0.0039 & 0.0928 $\pm$ 0.0042 \\
Reverse KL & \textbf{0.1608 $\pm$ 0.0106} & \textbf{0.1769 $\pm$ 0.0076} & \textbf{0.1662 $\pm$ 0.0087} & \textbf{0.1648 $\pm$ 0.0087} \\
Pearson $\chi^2$ & 0.1023 $\pm$ 0.0031 & 0.1039 $\pm$ 0.0025 & 0.1050 $\pm$ 0.0025 & 0.1048 $\pm$ 0.0028 \\
Squared Hellinger & 0.0898 $\pm$ 0.0041 & 0.0926 $\pm$ 0.0033 & 0.0932 $\pm$ 0.0027 & 0.0937 $\pm$ 0.0012 \\
Jensen--Shannon & 0.0971 $\pm$ 0.0044 & 0.1026 $\pm$ 0.0021 & 0.1046 $\pm$ 0.0024 & 0.1044 $\pm$ 0.0022 \\
Total variation & \underline{0.1405 $\pm$ 0.0061} & \underline{0.1477 $\pm$ 0.0056} & \underline{0.1499 $\pm$ 0.0059} & \underline{0.1492 $\pm$ 0.0039} \\
\bottomrule
\end{tabular}
\caption{Staged f-RPO Spearman $\rho$ across divergence choices and observed ranking depths on the test split. Values are mean $\pm$ sample standard deviation over five seeds. Best results are bold and second-best results are underlined.}
\label{tab:frpo-divergence-spearman-test}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Divergence & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
KL & 0.2710 $\pm$ 0.0047 & 0.2726 $\pm$ 0.0062 & 0.2732 $\pm$ 0.0045 & 0.2694 $\pm$ 0.0065 \\
Reverse KL & \textbf{0.2921 $\pm$ 0.0052} & \textbf{0.2938 $\pm$ 0.0049} & \textbf{0.2900 $\pm$ 0.0027} & \textbf{0.2894 $\pm$ 0.0023} \\
Pearson $\chi^2$ & \underline{0.2791 $\pm$ 0.0043} & 0.2748 $\pm$ 0.0031 & 0.2780 $\pm$ 0.0036 & 0.2770 $\pm$ 0.0059 \\
Squared Hellinger & 0.2775 $\pm$ 0.0041 & 0.2797 $\pm$ 0.0035 & \underline{0.2808 $\pm$ 0.0031} & \underline{0.2808 $\pm$ 0.0015} \\
Jensen--Shannon & \underline{0.2791 $\pm$ 0.0033} & 0.2775 $\pm$ 0.0049 & 0.2791 $\pm$ 0.0027 & 0.2797 $\pm$ 0.0035 \\
Total variation & 0.2786 $\pm$ 0.0040 & \underline{0.2808 $\pm$ 0.0036} & 0.2786 $\pm$ 0.0023 & 0.2780 $\pm$ 0.0041 \\
\bottomrule
\end{tabular}
\caption{Staged f-RPO Top-1 accuracy across divergence choices and observed ranking depths on the test split. Values are mean $\pm$ sample standard deviation over five seeds. Best results are bold and second-best results are underlined.}
\label{tab:frpo-divergence-top1-test}
\end{table}


==> test_method_topk_tables.tex <==
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lrrrr}
% \toprule
% Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
% \midrule
% Baseline & 0.0314 & 0.0314 & 0.0314 & 0.0314 \\
% \midrule
% DPO & 0.1612 $\pm$ 0.0043 & 0.1695 $\pm$ 0.0058 & 0.1956 $\pm$ 0.0067 & 0.1914 $\pm$ 0.0042 \\
% PL-DPO & 0.0967 $\pm$ 0.0050 & 0.1031 $\pm$ 0.0047 & 0.1104 $\pm$ 0.0045 & 0.1131 $\pm$ 0.0037 \\
% Legacy f-RPO-TV & 0.1289 $\pm$ 0.0067 & 0.1438 $\pm$ 0.0083 & 0.1478 $\pm$ 0.0055 & 0.1474 $\pm$ 0.0051 \\
% Staged f-RPO-TV & 0.1405 $\pm$ 0.0061 & 0.1477 $\pm$ 0.0056 & 0.1499 $\pm$ 0.0059 & 0.1492 $\pm$ 0.0039 \\
% Mallows-RCPO & 0.1300 $\pm$ 0.0049 & 0.1287 $\pm$ 0.0038 & 0.1307 $\pm$ 0.0053 & 0.1315 $\pm$ 0.0051 \\
% Mallows-TV & 0.1284 $\pm$ 0.0030 & 0.1276 $\pm$ 0.0024 & 0.1312 $\pm$ 0.0063 & 0.1302 $\pm$ 0.0057 \\
% \bottomrule
% \end{tabular}
% \caption{Global ranking results on the test split. Trained cells report mean $\pm$ sample standard deviation across five seeds.}
% \label{tab:spearman-test-method-topk}
% \end{table}

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lrrrr}
% \toprule
% Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
% \midrule
% Baseline & 0.2385 & 0.2385 & 0.2385 & 0.2385 \\
% \midrule
% DPO & 0.2965 $\pm$ 0.0076 & 0.2976 $\pm$ 0.0040 & 0.3019 $\pm$ 0.0056 & 0.3003 $\pm$ 0.0012 \\
% PL-DPO & 0.2791 $\pm$ 0.0027 & 0.2775 $\pm$ 0.0015 & 0.2791 $\pm$ 0.0019 & 0.2824 $\pm$ 0.0035 \\
% Legacy f-RPO-TV & 0.2786 $\pm$ 0.0040 & 0.2791 $\pm$ 0.0066 & 0.2797 $\pm$ 0.0045 & 0.2808 $\pm$ 0.0041 \\
% Staged f-RPO-TV & 0.2786 $\pm$ 0.0040 & 0.2808 $\pm$ 0.0036 & 0.2786 $\pm$ 0.0023 & 0.2780 $\pm$ 0.0041 \\
% Mallows-RCPO & 0.2851 $\pm$ 0.0065 & 0.2835 $\pm$ 0.0062 & 0.2829 $\pm$ 0.0071 & 0.2846 $\pm$ 0.0043 \\
% Mallows-TV & 0.2840 $\pm$ 0.0056 & 0.2835 $\pm$ 0.0071 & 0.2856 $\pm$ 0.0065 & 0.2856 $\pm$ 0.0068 \\
% \bottomrule
% \end{tabular}
% \caption{Top-1 selection results on the test split. Trained cells report mean $\pm$ sample standard deviation across five seeds.}
% \label{tab:top1-test-method-topk}
% \end{table}
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
Baseline & 0.0314 & 0.0314 & 0.0314 & 0.0314 \\
\midrule
PL-DPO & 0.0967 $\pm$ 0.0050 & 0.1031 $\pm$ 0.0047 & 0.1104 $\pm$ 0.0045 & 0.1131 $\pm$ 0.0037 \\
Legacy f-RPO-TV & 0.1289 $\pm$ 0.0067 & \underline{0.1438 $\pm$ 0.0083} & \underline{0.1478 $\pm$ 0.0055} & \underline{0.1474 $\pm$ 0.0051} \\
Staged f-RPO-TV & \textbf{0.1405 $\pm$ 0.0061} & \textbf{0.1477 $\pm$ 0.0056} & \textbf{0.1499 $\pm$ 0.0059} & \textbf{0.1492 $\pm$ 0.0039} \\
Mallows-RCPO & \underline{0.1300 $\pm$ 0.0049} & 0.1287 $\pm$ 0.0038 & 0.1307 $\pm$ 0.0053 & 0.1315 $\pm$ 0.0051 \\
Mallows-TV & 0.1284 $\pm$ 0.0030 & 0.1276 $\pm$ 0.0024 & 0.1312 $\pm$ 0.0063 & 0.1302 $\pm$ 0.0057 \\
\bottomrule
\end{tabular}
\caption{Global ranking results on the test split, excluding DPO. Trained cells report mean $\pm$ sample standard deviation across five seeds. Best results are bold and second-best results are underlined.}
\label{tab:spearman-test-method-topk-no-dpo}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
Baseline & 0.2385 & 0.2385 & 0.2385 & 0.2385 \\
\midrule
PL-DPO & 0.2791 $\pm$ 0.0027 & 0.2775 $\pm$ 0.0015 & 0.2791 $\pm$ 0.0019 & 0.2824 $\pm$ 0.0035 \\
Legacy f-RPO-TV & 0.2786 $\pm$ 0.0040 & 0.2791 $\pm$ 0.0066 & 0.2797 $\pm$ 0.0045 & 0.2808 $\pm$ 0.0041 \\
Staged f-RPO-TV & 0.2786 $\pm$ 0.0040 & \underline{0.2808 $\pm$ 0.0036} & 0.2786 $\pm$ 0.0023 & 0.2780 $\pm$ 0.0041 \\
Mallows-RCPO & \textbf{0.2851 $\pm$ 0.0065} & \textbf{0.2835 $\pm$ 0.0062} & \underline{0.2829 $\pm$ 0.0071} & \underline{0.2846 $\pm$ 0.0043} \\
Mallows-TV & \underline{0.2840 $\pm$ 0.0056} & \textbf{0.2835 $\pm$ 0.0071} & \textbf{0.2856 $\pm$ 0.0065} & \textbf{0.2856 $\pm$ 0.0068} \\
\bottomrule
\end{tabular}
\caption{Top-1 selection results on the test split, excluding DPO. Trained cells report mean $\pm$ sample standard deviation across five seeds. Best results are bold and second-best results are underlined.}
\label{tab:top1-test-method-topk-no-dpo}
\end{table}

==> top_k_test_ultra_feedback_prelim.tex <==
% Requires: \usepackage{booktabs,graphicx}
\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
Setting & Spearman $\uparrow$ & Kendall $\uparrow$ & Pairwise $\uparrow$ & Top-1 $\uparrow$ & Exact $\uparrow$ & Rank MAE $\downarrow$ & Norm. entropy & Effective choices \\
\midrule
Baseline & 0.0314 & 0.0320 & 0.5160 & 0.2385 & 0.0244 & 1.5631 & 0.9614 & 4.7278 \\
\midrule
$k=2$ & 0.1300 $\pm$ 0.0049 & 0.1064 $\pm$ 0.0039 & 0.5532 $\pm$ 0.0019 & \textbf{0.2851 $\pm$ 0.0065} & 0.0276 $\pm$ 0.0023 & 1.4526 $\pm$ 0.0065 & 0.9570 $\pm$ 0.0006 & 4.7017 $\pm$ 0.0035 \\
$k=3$ & 0.1287 $\pm$ 0.0038 & 0.1057 $\pm$ 0.0035 & 0.5528 $\pm$ 0.0018 & 0.2835 $\pm$ 0.0062 & \textbf{0.0282 $\pm$ 0.0015} & 1.4545 $\pm$ 0.0052 & 0.9570 $\pm$ 0.0005 & 4.7011 $\pm$ 0.0032 \\
$k=4$ & 0.1307 $\pm$ 0.0053 & 0.1072 $\pm$ 0.0044 & 0.5536 $\pm$ 0.0022 & 0.2829 $\pm$ 0.0071 & 0.0282 $\pm$ 0.0015 & 1.4528 $\pm$ 0.0058 & 0.9570 $\pm$ 0.0006 & 4.7013 $\pm$ 0.0037 \\
$k=5$ (full) & \textbf{0.1315 $\pm$ 0.0051} & \textbf{0.1075 $\pm$ 0.0045} & \textbf{0.5538 $\pm$ 0.0022} & 0.2846 $\pm$ 0.0043 & 0.0282 $\pm$ 0.0015 & \textbf{1.4513 $\pm$ 0.0044} & 0.9570 $\pm$ 0.0005 & 4.7014 $\pm$ 0.0031 \\
\bottomrule
\end{tabular}%
}
\caption{Mallows-RMJ RCPO ranking and candidate-diversity results on the test split. Seeded values are mean $\pm$ sample standard deviation.}
\label{tab:mallows_rcpo-test-topk}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
Setting & Spearman $\uparrow$ & Kendall $\uparrow$ & Pairwise $\uparrow$ & Top-1 $\uparrow$ & Exact $\uparrow$ & Rank MAE $\downarrow$ & Norm. entropy & Effective choices \\
\midrule
Baseline & 0.0314 & 0.0320 & 0.5160 & 0.2385 & 0.0244 & 1.5631 & 0.9614 & 4.7278 \\
\midrule
$k=2$ & 0.1284 $\pm$ 0.0030 & 0.1054 $\pm$ 0.0023 & 0.5527 $\pm$ 0.0011 & 0.2840 $\pm$ 0.0056 & \textbf{0.0282 $\pm$ 0.0015} & 1.4532 $\pm$ 0.0046 & 0.9571 $\pm$ 0.0005 & 4.7019 $\pm$ 0.0031 \\
$k=3$ & 0.1276 $\pm$ 0.0024 & 0.1043 $\pm$ 0.0010 & 0.5521 $\pm$ 0.0005 & 0.2835 $\pm$ 0.0071 & 0.0282 $\pm$ 0.0015 & 1.4552 $\pm$ 0.0044 & 0.9570 $\pm$ 0.0006 & 4.7014 $\pm$ 0.0036 \\
$k=4$ & \textbf{0.1312 $\pm$ 0.0063} & \textbf{0.1072 $\pm$ 0.0048} & \textbf{0.5536 $\pm$ 0.0024} & \textbf{0.2856 $\pm$ 0.0065} & 0.0282 $\pm$ 0.0015 & \textbf{1.4519 $\pm$ 0.0059} & 0.9570 $\pm$ 0.0006 & 4.7012 $\pm$ 0.0034 \\
$k=5$ (full) & 0.1302 $\pm$ 0.0057 & 0.1071 $\pm$ 0.0045 & 0.5536 $\pm$ 0.0023 & 0.2856 $\pm$ 0.0068 & 0.0282 $\pm$ 0.0015 & 1.4534 $\pm$ 0.0066 & 0.9570 $\pm$ 0.0004 & 4.7013 $\pm$ 0.0027 \\
\bottomrule
\end{tabular}%
}
\caption{Mallows-TV RCPO ranking and candidate-diversity results on the test split. Seeded values are mean $\pm$ sample standard deviation.}
\label{tab:mallows_tv-test-topk}
\end{table*}




==> top_k_train_ultra_feedback_prelim.tex <==
% Requires: \usepackage{booktabs,graphicx}
\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
Setting & Spearman $\uparrow$ & Kendall $\uparrow$ & Pairwise $\uparrow$ & Top-1 $\uparrow$ & Exact $\uparrow$ & Rank MAE $\downarrow$ & Norm. entropy & Effective choices \\
\midrule
Baseline & 0.0285 & 0.0277 & 0.5139 & 0.2119 & 0.0125 & 1.5599 & 0.9631 & 4.7421 \\
\midrule
$k=2$ & 0.1650 $\pm$ 0.0025 & 0.1386 $\pm$ 0.0028 & 0.5693 $\pm$ 0.0014 & \textbf{0.2897 $\pm$ 0.0029} & \textbf{0.0189 $\pm$ 0.0005} & 1.4135 $\pm$ 0.0025 & 0.9583 $\pm$ 0.0005 & 4.7115 $\pm$ 0.0028 \\
$k=3$ & 0.1634 $\pm$ 0.0036 & 0.1376 $\pm$ 0.0031 & 0.5688 $\pm$ 0.0016 & 0.2881 $\pm$ 0.0031 & 0.0186 $\pm$ 0.0013 & 1.4161 $\pm$ 0.0029 & 0.9582 $\pm$ 0.0004 & 4.7109 $\pm$ 0.0024 \\
$k=4$ & 0.1655 $\pm$ 0.0054 & 0.1389 $\pm$ 0.0050 & 0.5694 $\pm$ 0.0025 & 0.2887 $\pm$ 0.0034 & 0.0179 $\pm$ 0.0020 & 1.4133 $\pm$ 0.0058 & 0.9582 $\pm$ 0.0005 & 4.7108 $\pm$ 0.0028 \\
$k=5$ (full) & \textbf{0.1659 $\pm$ 0.0054} & \textbf{0.1394 $\pm$ 0.0049} & \textbf{0.5697 $\pm$ 0.0024} & 0.2891 $\pm$ 0.0033 & 0.0181 $\pm$ 0.0017 & \textbf{1.4132 $\pm$ 0.0060} & 0.9582 $\pm$ 0.0004 & 4.7109 $\pm$ 0.0024 \\
\bottomrule
\end{tabular}%
}
\caption{Mallows-RMJ RCPO ranking and candidate-diversity results on the train split. Seeded values are mean $\pm$ sample standard deviation.}
\label{tab:mallows_rcpo-train-topk}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr}
\toprule
Setting & Spearman $\uparrow$ & Kendall $\uparrow$ & Pairwise $\uparrow$ & Top-1 $\uparrow$ & Exact $\uparrow$ & Rank MAE $\downarrow$ & Norm. entropy & Effective choices \\
\midrule
Baseline & 0.0285 & 0.0277 & 0.5139 & 0.2119 & 0.0125 & 1.5599 & 0.9631 & 4.7421 \\
\midrule
$k=2$ & 0.1643 $\pm$ 0.0025 & 0.1382 $\pm$ 0.0024 & 0.5691 $\pm$ 0.0012 & \textbf{0.2896 $\pm$ 0.0027} & \textbf{0.0186 $\pm$ 0.0014} & 1.4146 $\pm$ 0.0018 & 0.9583 $\pm$ 0.0004 & 4.7115 $\pm$ 0.0024 \\
$k=3$ & 0.1621 $\pm$ 0.0036 & 0.1365 $\pm$ 0.0034 & 0.5682 $\pm$ 0.0017 & 0.2888 $\pm$ 0.0033 & 0.0185 $\pm$ 0.0016 & 1.4175 $\pm$ 0.0038 & 0.9582 $\pm$ 0.0004 & 4.7110 $\pm$ 0.0028 \\
$k=4$ & 0.1655 $\pm$ 0.0041 & 0.1389 $\pm$ 0.0038 & 0.5695 $\pm$ 0.0019 & 0.2884 $\pm$ 0.0026 & 0.0186 $\pm$ 0.0014 & 1.4132 $\pm$ 0.0042 & 0.9581 $\pm$ 0.0004 & 4.7106 $\pm$ 0.0024 \\
$k=5$ (full) & \textbf{0.1661 $\pm$ 0.0049} & \textbf{0.1395 $\pm$ 0.0046} & \textbf{0.5698 $\pm$ 0.0023} & 0.2890 $\pm$ 0.0029 & 0.0178 $\pm$ 0.0022 & \textbf{1.4127 $\pm$ 0.0061} & 0.9582 $\pm$ 0.0003 & 4.7107 $\pm$ 0.0020 \\
\bottomrule
\end{tabular}%
}
\caption{Mallows-TV RCPO ranking and candidate-diversity results on the train split. Seeded values are mean $\pm$ sample standard deviation.}
\label{tab:mallows_tv-train-topk}
\end{table*}



==> train_fdiv_method_topk_tables.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Divergence & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
KL & 0.1250 $\pm$ 0.0030 & 0.1297 $\pm$ 0.0035 & 0.1314 $\pm$ 0.0045 & 0.1304 $\pm$ 0.0047 \\
Reverse KL & \textbf{0.2020 $\pm$ 0.0059} & \textbf{0.2153 $\pm$ 0.0054} & \underline{0.2035 $\pm$ 0.0069} & \underline{0.2027 $\pm$ 0.0070} \\
Pearson $\chi^2$ & 0.1476 $\pm$ 0.0021 & 0.1516 $\pm$ 0.0032 & 0.1540 $\pm$ 0.0026 & 0.1541 $\pm$ 0.0030 \\
Squared Hellinger & 0.1256 $\pm$ 0.0035 & 0.1286 $\pm$ 0.0032 & 0.1293 $\pm$ 0.0014 & 0.1288 $\pm$ 0.0017 \\
Jensen--Shannon & 0.1375 $\pm$ 0.0022 & 0.1448 $\pm$ 0.0028 & 0.1473 $\pm$ 0.0027 & 0.1471 $\pm$ 0.0033 \\
Total variation & \underline{0.2010 $\pm$ 0.0059} & \underline{0.2115 $\pm$ 0.0050} & \textbf{0.2137 $\pm$ 0.0045} & \textbf{0.2128 $\pm$ 0.0031} \\
\bottomrule
\end{tabular}
\caption{Staged f-RPO Spearman $\rho$ across divergence choices and observed ranking depths on the train split. Values are mean $\pm$ sample standard deviation over five seeds. Best results are bold and second-best results are underlined.}
\label{tab:frpo-divergence-spearman-train}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Divergence & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
KL & 0.2488 $\pm$ 0.0029 & 0.2453 $\pm$ 0.0020 & 0.2439 $\pm$ 0.0015 & 0.2438 $\pm$ 0.0020 \\
Reverse KL & \underline{0.2683 $\pm$ 0.0016} & \underline{0.2650 $\pm$ 0.0047} & \underline{0.2601 $\pm$ 0.0020} & \underline{0.2607 $\pm$ 0.0007} \\
Pearson $\chi^2$ & 0.2595 $\pm$ 0.0025 & 0.2539 $\pm$ 0.0018 & 0.2542 $\pm$ 0.0018 & 0.2542 $\pm$ 0.0020 \\
Squared Hellinger & 0.2534 $\pm$ 0.0026 & 0.2485 $\pm$ 0.0021 & 0.2479 $\pm$ 0.0027 & 0.2472 $\pm$ 0.0017 \\
Jensen--Shannon & 0.2568 $\pm$ 0.0039 & 0.2528 $\pm$ 0.0034 & 0.2530 $\pm$ 0.0031 & 0.2536 $\pm$ 0.0033 \\
Total variation & \textbf{0.2737 $\pm$ 0.0033} & \textbf{0.2712 $\pm$ 0.0014} & \textbf{0.2704 $\pm$ 0.0022} & \textbf{0.2694 $\pm$ 0.0027} \\
\bottomrule
\end{tabular}
\caption{Staged f-RPO Top-1 accuracy across divergence choices and observed ranking depths on the train split. Values are mean $\pm$ sample standard deviation over five seeds. Best results are bold and second-best results are underlined.}
\label{tab:frpo-divergence-top1-train}
\end{table}


==> train_method_topk_tables.tex <==
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lrrrr}
% \toprule
% Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
% \midrule
% Baseline & 0.0285 & 0.0285 & 0.0285 & 0.0285 \\
% \midrule
% DPO & 0.3122 $\pm$ 0.0055 & 0.3232 $\pm$ 0.0071 & 0.3417 $\pm$ 0.0068 & 0.3404 $\pm$ 0.0036 \\
% PL-DPO & 0.1321 $\pm$ 0.0031 & 0.1422 $\pm$ 0.0046 & 0.1543 $\pm$ 0.0064 & 0.1555 $\pm$ 0.0053 \\
% Legacy f-RPO-TV & 0.1842 $\pm$ 0.0070 & 0.2056 $\pm$ 0.0048 & 0.2110 $\pm$ 0.0050 & 0.2114 $\pm$ 0.0038 \\
% Staged f-RPO-TV & 0.2010 $\pm$ 0.0059 & 0.2115 $\pm$ 0.0050 & 0.2137 $\pm$ 0.0045 & 0.2128 $\pm$ 0.0031 \\
% Mallows-RCPO & 0.1650 $\pm$ 0.0025 & 0.1634 $\pm$ 0.0036 & 0.1655 $\pm$ 0.0054 & 0.1659 $\pm$ 0.0054 \\
% Mallows-TV & 0.1643 $\pm$ 0.0025 & 0.1621 $\pm$ 0.0036 & 0.1655 $\pm$ 0.0041 & 0.1661 $\pm$ 0.0049 \\
% \bottomrule
% \end{tabular}
% \caption{Global ranking results on the train split. Trained cells report mean $\pm$ sample standard deviation across five seeds.}
% \label{tab:spearman-train-method-topk}
% \end{table}

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lrrrr}
% \toprule
% Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
% \midrule
% Baseline & 0.2119 & 0.2119 & 0.2119 & 0.2119 \\
% \midrule
% DPO & 0.3650 $\pm$ 0.0031 & 0.3469 $\pm$ 0.0064 & 0.3454 $\pm$ 0.0059 & 0.3432 $\pm$ 0.0039 \\
% PL-DPO & 0.2597 $\pm$ 0.0011 & 0.2537 $\pm$ 0.0019 & 0.2558 $\pm$ 0.0023 & 0.2553 $\pm$ 0.0019 \\
% Legacy f-RPO-TV & 0.2769 $\pm$ 0.0039 & 0.2762 $\pm$ 0.0044 & 0.2755 $\pm$ 0.0026 & 0.2751 $\pm$ 0.0035 \\
% Staged f-RPO-TV & 0.2737 $\pm$ 0.0033 & 0.2712 $\pm$ 0.0014 & 0.2704 $\pm$ 0.0022 & 0.2694 $\pm$ 0.0027 \\
% Mallows-RCPO & 0.2897 $\pm$ 0.0029 & 0.2881 $\pm$ 0.0031 & 0.2887 $\pm$ 0.0034 & 0.2891 $\pm$ 0.0033 \\
% Mallows-TV & 0.2896 $\pm$ 0.0027 & 0.2888 $\pm$ 0.0033 & 0.2884 $\pm$ 0.0026 & 0.2890 $\pm$ 0.0029 \\
% \bottomrule
% \end{tabular}
% \caption{Top-1 selection results on the train split. Trained cells report mean $\pm$ sample standard deviation across five seeds.}
% \label{tab:top1-train-method-topk}
% \end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
Baseline & 0.0285 & 0.0285 & 0.0285 & 0.0285 \\
\midrule
PL-DPO & 0.1321 $\pm$ 0.0031 & 0.1422 $\pm$ 0.0046 & 0.1543 $\pm$ 0.0064 & 0.1555 $\pm$ 0.0053 \\
Legacy f-RPO-TV & \underline{0.1842 $\pm$ 0.0070} & \underline{0.2056 $\pm$ 0.0048} & \underline{0.2110 $\pm$ 0.0050} & \underline{0.2114 $\pm$ 0.0038} \\
Staged f-RPO-TV & \textbf{0.2010 $\pm$ 0.0059} & \textbf{0.2115 $\pm$ 0.0050} & \textbf{0.2137 $\pm$ 0.0045} & \textbf{0.2128 $\pm$ 0.0031} \\
Mallows-RCPO & 0.1650 $\pm$ 0.0025 & 0.1634 $\pm$ 0.0036 & 0.1655 $\pm$ 0.0054 & 0.1659 $\pm$ 0.0054 \\
Mallows-TV & 0.1643 $\pm$ 0.0025 & 0.1621 $\pm$ 0.0036 & 0.1655 $\pm$ 0.0041 & 0.1661 $\pm$ 0.0049 \\
\bottomrule
\end{tabular}
\caption{Global ranking results on the train split, excluding DPO. Trained cells report mean $\pm$ sample standard deviation across five seeds. Best results are bold and second-best results are underlined.}
\label{tab:spearman-train-method-topk-no-dpo}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Method & $k=2$ & $k=3$ & $k=4$ & $k=5$ (full) \\
\midrule
Baseline & 0.2119 & 0.2119 & 0.2119 & 0.2119 \\
\midrule
PL-DPO & 0.2597 $\pm$ 0.0011 & 0.2537 $\pm$ 0.0019 & 0.2558 $\pm$ 0.0023 & 0.2553 $\pm$ 0.0019 \\
Legacy f-RPO-TV & 0.2769 $\pm$ 0.0039 & 0.2762 $\pm$ 0.0044 & 0.2755 $\pm$ 0.0026 & 0.2751 $\pm$ 0.0035 \\
Staged f-RPO-TV & 0.2737 $\pm$ 0.0033 & 0.2712 $\pm$ 0.0014 & 0.2704 $\pm$ 0.0022 & 0.2694 $\pm$ 0.0027 \\
Mallows-RCPO & \textbf{0.2897 $\pm$ 0.0029} & \underline{0.2881 $\pm$ 0.0031} & \textbf{0.2887 $\pm$ 0.0034} & \textbf{0.2891 $\pm$ 0.0033} \\
Mallows-TV & \underline{0.2896 $\pm$ 0.0027} & \textbf{0.2888 $\pm$ 0.0033} & \underline{0.2884 $\pm$ 0.0026} & \underline{0.2890 $\pm$ 0.0029} \\
\bottomrule
\end{tabular}
\caption{Top-1 selection results on the train split, excluding DPO. Trained cells report mean $\pm$ sample standard deviation across five seeds. Best results are bold and second-best results are underlined.}
\label{tab:top1-train-method-topk-no-dpo}
\end{table}

